Distributions and Physical Properties of Molecular Clouds in the G24 Region of the Milky Way

We report the spatial distribution and physical characteristics of molecular clouds in the G24 region, which is located near the intersection of the Milky Way's Galactic bar with the Norma arm and the 3 kpc arm. Utilizing molecular line data from the Milky Way Imaging Scroll Painting (MWISP) project, including $^{12}$CO, $^{13}$CO, and C$^{18}$O, along with our own observations of HCO$^{+}$ line using the Purple Mountain Observatory (PMO) 13.7 m telescope, we have revealed the complex architecture of molecular clouds in the G24 region. Seven giant molecular clouds, each with a mass exceeding $10^4$ $M_\odot$ and a typical H$_2$ column density of $10^{21}$ cm$^{-2}$, have been identified through observations of CO and its isotopes. The conversion factor $X_{\text{CO}}$ for the G24 region is estimated to be 8.25 $\times$ 10$^{19}$ cm$^{-2}$ (K km s$^{-1}$)$^{-1}$, aligning with the typical values observed in other regions. Adopting the GaussClumps algorithm, we have identified a total of 257, 201, and 110 clumps in $^{12}$CO, $^{13}$CO and C$^{18}$O within G24 region, respectively. The derived physical properties (including effective radius, mass, and virial parameter) indicate that the majority of these clumps are gravitationally bound, with a subset possessing the potential to form massive stars. Examination of gas infall activities within these clumps further suggests ongoing massive star formation. The complex physical and kinematic environment, shaped by the G24 region's unique location within the Milky Way, has limited the clear detection of gas outflows.

==> the_parameters_of_12CO_clumps.tex <==
\begin{longrotatetable}
\addtolength{\tabcolsep}{-1.5pt}
\begin{deluxetable*}{ccccccccccccccccccccc}
\tablecaption{The parameters of $^{12}$CO clumps}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{Number} & \colhead{Source} & \colhead{$V_{\text{lsr}}$} & \colhead{$\Delta v$} & \colhead{$\theta_{\text{a}}$} & \colhead{$\theta_{\text{b}}$} & \colhead{$\theta_{\text{fwhm}}$} & \colhead{P.A.} & \colhead{Distance} & \colhead{$R_{\text{GC}}$} & \colhead{$T_{\text{ex}}$} & \colhead{log($N_{\text{H$_2$}}$)} & \colhead{$R_{\text{eff}}$} & \colhead{log($M_{\text{clump}}$)} & \colhead{log($M_{\text{vir}}$)} & \colhead{$\alpha_{\text{vir}}$} & \colhead{log($\Sigma$)} & \colhead{log($n_{\text{H$_2$}}$)} & \colhead{$\Delta v_{\text{th}}$} & \colhead{$\Delta v_{\text{nth}}$} & \colhead{Potential} \\
\colhead{} & \colhead{} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{($\arcsec$)} & \colhead{($\arcsec$)} & \colhead{($\arcsec$)} & \colhead{($\arcdeg$)} & \colhead{(kpc)} & \colhead{(kpc)} & \colhead{(K)} & \colhead{(cm$^{-2}$)} & \colhead{(pc)} & \colhead{($M_{\sun}$)} & \colhead{($M_{\sun}$)} & \colhead{} & \colhead{($M_{\sun}$ pc$^{-2}$)} & \colhead{(cm$^{-3}$)} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{}
\decimalcolnumbers
}
\startdata
1   & MWISP G24.469$+$0.483 & 103.48 & 4.05 & 126 & 167 & 142 & 75  & 5.66 & 3.81 & 14.3 & 21.6 & 1.9 & 3.2 & 3.8 & 4.2  & 2.1 & 2.4 & 0.15 & 4.05 &  \\
2   & MWISP G24.506$-$0.234 & 99.83  & 2.94 & 91  & 167 & 113 & 115 & 5.71 & 3.79 & 15.4 & 21.5 & 1.6 & 3.0 & 3.5 & 3.1  & 2.1 & 2.2 & 0.16 & 2.94 &  \\
3   & MWISP G24.458$+$0.502 & 100.63 & 2.39 & 142 & 172 & 155 & 10  & 5.59 & 3.84 & 12.8 & 21.3 & 2.0 & 3.0 & 3.4 & 2.7  & 1.8 & 1.8 & 0.14 & 2.39 &  \\
4   & MWISP G24.555$-$0.235 & 98.56  & 2.05 & 128 & 202 & 152 & 116 & 5.67 & 3.81 & 15.1 & 21.3 & 2.1 & 3.0 & 3.3 & 1.8  & 1.9 & 1.7 & 0.16 & 2.04 &  \\
5   & MWISP G24.670$-$0.156 & 113.17 & 2.97 & 97  & 244 & 128 & 108 & 6.94 & 3.43 & 14.0 & 21.4 & 2.5 & 3.3 & 3.7 & 2.4  & 2.0 & 1.9 & 0.15 & 2.97 &  \\
6   & MWISP G24.788$+$0.094 & 112.34 & 2.19 & 106 & 150 & 122 & 118 & 6.63 & 3.50 & 17.0 & 21.4 & 1.9 & 3.0 & 3.3 & 1.7  & 2.0 & 1.8 & 0.17 & 2.18 &  \\
7   & MWISP G24.723$+$0.081 & 109.85 & 1.94 & 66  & 115 & 81  & -11 & 6.42 & 3.55 & 13.4 & 21.2 & 1.1 & 2.5 & 2.9 & 2.8  & 1.9 & 2.2 & 0.15 & 1.93 &  \\
8   & MWISP G24.468$+$0.187 & 119.20 & 2.19 & 89  & 129 & 103 & 57  & 7.23 & 3.38 & 11.1 & 21.2 & 1.7 & 2.7 & 3.2 & 3.2  & 1.8 & 1.9 & 0.13 & 2.19 &  \\
9   & MWISP G24.537$-$0.210 & 101.26 & 2.75 & 72  & 167 & 93  & 10  & 5.78 & 3.76 & 18.5 & 21.6 & 1.4 & 2.9 & 3.3 & 2.5  & 2.2 & 2.3 & 0.17 & 2.74 &  \\
10  & MWISP G24.764$+$0.072 & 110.28 & 2.08 & 161 & 239 & 189 & 156 & 6.44 & 3.55 & 18.3 & 21.4 & 3.0 & 3.4 & 3.4 & 1.0  & 2.0 & 1.4 & 0.17 & 2.07 &  \\
11  & MWISP G24.225$+$0.231 & 114.11 & 1.98 & 137 & 284 & 175 & 39  & 7.21 & 3.35 & 10.7 & 21.1 & 3.3 & 3.2 & 3.4 & 1.8  & 1.6 & 1.2 & 0.13 & 1.98 &  \\
12  & MWISP G24.503$+$0.454 & 104.10 & 1.59 & 101 & 140 & 116 & -11 & 5.68 & 3.80 & 12.8 & 21.1 & 1.5 & 2.5 & 2.9 & 2.2  & 1.7 & 1.8 & 0.14 & 1.58 &  \\
13  & MWISP G24.412$+$0.077 & 112.88 & 1.91 & 132 & 263 & 166 & 104 & 6.92 & 3.41 & 21.7 & 21.5 & 3.0 & 3.5 & 3.4 & 0.8  & 2.0 & 1.3 & 0.19 & 1.90 &  \\
14  & MWISP G24.434$+$0.266 & 117.63 & 1.29 & 99  & 148 & 117 & 108 & 7.17 & 3.38 & 9.9  & 20.9 & 1.9 & 2.5 & 2.8 & 2.0  & 1.5 & 1.3 & 0.13 & 1.28 &  \\
15  & MWISP G24.733$+$0.141 & 108.57 & 2.24 & 93  & 148 & 111 & 118 & 5.16 & 4.08 & 18.4 & 21.5 & 1.3 & 2.8 & 3.1 & 2.2  & 2.1 & 2.1 & 0.17 & 2.23 &  \\
16  & MWISP G24.486$-$0.045 & 108.75 & 2.24 & 129 & 221 & 158 & 113 & 6.82 & 3.43 & 11.7 & 21.2 & 2.7 & 3.1 & 3.4 & 2.2  & 1.8 & 1.5 & 0.14 & 2.24 &  \\
17  & MWISP G24.837$-$0.026 & 104.45 & 1.82 & 156 & 157 & 156 & 0   & 5.99 & 3.70 & 14.6 & 21.3 & 2.2 & 3.0 & 3.2 & 1.6  & 1.8 & 1.6 & 0.15 & 1.81 &  \\
18  & MWISP G24.485$-$0.040 & 111.27 & 2.25 & 134 & 168 & 148 & 90  & 6.67 & 3.46 & 9.3  & 21.1 & 2.3 & 2.8 & 3.4 & 3.5  & 1.6 & 1.7 & 0.12 & 2.25 &  \\
19  & MWISP G24.508$+$0.465 & 102.67 & 1.14 & 68  & 169 & 89  & 148 & 5.65 & 3.81 & 13.7 & 21.0 & 1.3 & 2.4 & 2.5 & 1.6  & 1.6 & 1.6 & 0.15 & 1.13 &  \\
20  & MWISP G24.762$+$0.081 & 107.94 & 2.20 & 153 & 181 & 165 & 2   & 5.55 & 3.88 & 18.6 & 21.5 & 2.1 & 3.2 & 3.3 & 1.5  & 2.0 & 1.7 & 0.17 & 2.19 &  \\
21  & MWISP G24.653$-$0.104 & 114.89 & 2.86 & 114 & 135 & 123 & 144 & 6.93 & 3.43 & 9.2  & 21.2 & 1.9 & 2.8 & 3.5 & 5.0  & 1.8 & 2.0 & 0.12 & 2.86 &  \\
22  & MWISP G24.453$-$0.285 & 96.65  & 1.94 & 114 & 169 & 133 & -6  & 5.48 & 3.89 & 15.4 & 21.3 & 1.7 & 2.8 & 3.1 & 1.9  & 1.9 & 1.8 & 0.16 & 1.93 &  \\
23  & MWISP G24.480$+$0.309 & 117.31 & 2.28 & 112 & 244 & 144 & 130 & 6.83 & 3.43 & 9.0  & 21.1 & 2.6 & 2.9 & 3.5 & 3.3  & 1.6 & 1.6 & 0.12 & 2.28 &  \\
24  & MWISP G24.428$+$0.128 & 116.04 & 2.58 & 147 & 254 & 180 & 89  & 7.23 & 3.38 & 15.4 & 21.4 & 3.3 & 3.5 & 3.7 & 1.4  & 2.0 & 1.5 & 0.16 & 2.58 &  \\
25  & MWISP G24.475$+$0.476 & 100.95 & 2.75 & 72  & 123 & 88  & 120 & 5.48 & 3.89 & 13.8 & 21.4 & 1.1 & 2.6 & 3.2 & 4.3  & 2.0 & 2.5 & 0.15 & 2.75 &  \\
26  & MWISP G24.858$+$0.053 & 108.89 & 3.11 & 88  & 202 & 114 & 93  & 5.38 & 3.97 & 15.4 & 21.5 & 1.6 & 3.0 & 3.5 & 3.3  & 2.1 & 2.3 & 0.16 & 3.11 &  \\
27  & MWISP G24.143$-$0.102 & 80.27  & 1.98 & 130 & 254 & 163 & 80  & 5.08 & 4.08 & 9.9  & 21.1 & 2.2 & 2.8 & 3.2 & 3.1  & 1.6 & 1.6 & 0.13 & 1.98 &  \\
28  & MWISP G24.526$+$0.329 & 113.13 & 2.54 & 268 & 403 & 316 & 127 & 6.56 & 3.49 & 8.7  & 21.1 & 5.2 & 3.5 & 3.8 & 2.1  & 1.6 & 1.1 & 0.12 & 2.54 &  \\
29  & MWISP G24.759$+$0.500 & 105.25 & 2.33 & 139 & 181 & 156 & 62  & 5.81 & 3.77 & 20.3 & 21.5 & 2.1 & 3.2 & 3.4 & 1.4  & 2.1 & 1.8 & 0.18 & 2.32 &  \\
30  & MWISP G24.208$-$0.259 & 93.63  & 1.96 & 104 & 134 & 116 & -10 & 5.25 & 3.99 & 6.3  & 20.7 & 1.4 & 2.1 & 3.0 & 9.1  & 1.3 & 2.0 & 0.10 & 1.96 &  \\
31  & MWISP G24.450$+$0.507 & 102.07 & 1.18 & 62  & 152 & 81  & 152 & 5.63 & 3.82 & 13.6 & 21.0 & 1.1 & 2.3 & 2.5 & 1.8  & 1.7 & 1.7 & 0.15 & 1.17 &  \\
32  & MWISP G24.365$+$0.043 & 119.67 & 2.12 & 133 & 246 & 165 & 103 & 7.32 & 3.36 & 15.8 & 21.4 & 3.1 & 3.4 & 3.5 & 1.2  & 1.9 & 1.4 & 0.16 & 2.11 &  \\
33  & MWISP G24.433$+$0.322 & 115.55 & 2.39 & 145 & 232 & 174 & 84  & 6.74 & 3.44 & 9.0  & 21.1 & 2.9 & 3.0 & 3.5 & 3.2  & 1.6 & 1.5 & 0.12 & 2.39 &  \\
34  & MWISP G24.949$+$0.471 & 111.27 & 2.09 & 112 & 137 & 123 & 0   & 6.39 & 3.58 & 14.4 & 21.3 & 1.8 & 2.9 & 3.2 & 2.1  & 1.9 & 1.8 & 0.15 & 2.08 &  \\
35  & MWISP G24.186$+$0.407 & 95.09  & 2.40 & 129 & 198 & 153 & 155 & 5.28 & 3.97 & 8.4  & 21.0 & 1.9 & 2.7 & 3.4 & 5.2  & 1.6 & 1.9 & 0.12 & 2.40 &  \\
36  & MWISP G24.215$-$0.053 & 91.72  & 2.24 & 103 & 132 & 115 & -39 & 5.29 & 3.97 & 11.0 & 21.2 & 1.4 & 2.5 & 3.2 & 4.2  & 1.8 & 2.1 & 0.13 & 2.24 &  \\
37  & MWISP G24.417$+$0.243 & 112.22 & 2.43 & 228 & 514 & 295 & 113 & 6.97 & 3.40 & 10.2 & 21.2 & 5.7 & 3.7 & 3.8 & 1.4  & 1.7 & 1.0 & 0.13 & 2.43 &  \\
38  & MWISP G24.632$-$0.120 & 112.38 & 2.79 & 170 & 206 & 186 & 89  & 6.75 & 3.46 & 11.2 & 21.3 & 3.0 & 3.3 & 3.7 & 2.7  & 1.8 & 1.6 & 0.13 & 2.79 &  \\
39  & MWISP G24.552$-$0.143 & 95.23  & 2.56 & 129 & 160 & 142 & -12 & 5.55 & 3.87 & 16.0 & 21.5 & 1.8 & 3.0 & 3.4 & 2.3  & 2.0 & 2.0 & 0.16 & 2.55 &  \\
40  & MWISP G24.508$-$0.109 & 94.92  & 2.77 & 125 & 205 & 151 & 58  & 5.53 & 3.87 & 12.2 & 21.3 & 2.0 & 3.0 & 3.5 & 3.3  & 1.9 & 2.0 & 0.14 & 2.77 &  \\
41  & MWISP G24.511$+$0.259 & 119.68 & 2.03 & 74  & 137 & 92  & 39  & 6.99 & 3.41 & 8.4  & 21.0 & 1.5 & 2.4 & 3.1 & 4.8  & 1.6 & 2.0 & 0.12 & 2.03 &  \\
42  & MWISP G24.462$+$0.490 & 105.24 & 3.03 & 73  & 117 & 87  & 152 & 5.70 & 3.79 & 14.3 & 21.5 & 1.1 & 2.7 & 3.3 & 4.4  & 2.1 & 2.6 & 0.15 & 3.03 &  \\
43  & MWISP G24.193$-$0.056 & 87.63  & 1.80 & 122 & 312 & 161 & 148 & 5.17 & 4.04 & 10.5 & 21.1 & 2.4 & 2.8 & 3.2 & 2.3  & 1.6 & 1.5 & 0.13 & 1.80 &  \\
44  & MWISP G24.373$+$0.042 & 115.56 & 1.74 & 150 & 251 & 182 & 137 & 7.25 & 3.37 & 15.9 & 21.3 & 3.3 & 3.4 & 3.3 & 0.9  & 1.8 & 1.1 & 0.16 & 1.73 &  \\
45  & MWISP G24.443$+$0.146 & 117.94 & 2.33 & 208 & 262 & 230 & -21 & 7.25 & 3.38 & 15.0 & 21.4 & 4.0 & 3.6 & 3.7 & 1.1  & 1.9 & 1.2 & 0.16 & 2.32 &  \\
46  & MWISP G24.801$+$0.103 & 106.34 & 2.87 & 111 & 285 & 146 & 115 & 6.04 & 3.68 & 15.8 & 21.5 & 2.5 & 3.3 & 3.6 & 2.0  & 2.0 & 1.8 & 0.16 & 2.87 &  \\
47  & MWISP G24.802$+$0.019 & 106.66 & 2.51 & 168 & 199 & 182 & 135 & 6.07 & 3.67 & 17.0 & 21.5 & 2.6 & 3.3 & 3.5 & 1.6  & 2.0 & 1.7 & 0.17 & 2.50 &  \\
48  & MWISP G24.141$+$0.248 & 113.79 & 1.26 & 120 & 272 & 155 & -29 & 7.39 & 3.33 & 12.2 & 21.0 & 3.1 & 3.0 & 3.0 & 1.0  & 1.5 & 0.9 & 0.14 & 1.25 &  \\
49  & MWISP G24.566$-$0.281 & 95.24  & 2.34 & 110 & 297 & 146 & -17 & 5.46 & 3.91 & 12.3 & 21.3 & 2.3 & 3.0 & 3.4 & 2.5  & 1.8 & 1.7 & 0.14 & 2.34 &  \\
50  & MWISP G24.375$+$0.042 & 117.44 & 1.50 & 158 & 242 & 187 & 117 & 7.30 & 3.37 & 15.9 & 21.2 & 3.4 & 3.3 & 3.2 & 0.8  & 1.8 & 1.0 & 0.16 & 1.49 &  \\
51  & MWISP G24.629$+$0.367 & 109.85 & 2.26 & 277 & 582 & 354 & 141 & 6.59 & 3.49 & 12.9 & 21.3 & 6.4 & 3.9 & 3.8 & 0.9  & 1.8 & 0.8 & 0.15 & 2.26 &  \\
52  & MWISP G24.548$-$0.243 & 100.00 & 1.80 & 69  & 87  & 76  & 57  & 5.72 & 3.79 & 14.8 & 21.3 & 0.8 & 2.3 & 2.7 & 2.7  & 2.0 & 2.4 & 0.16 & 1.79 &  \\
53  & MWISP G24.300$-$0.150 & 101.11 & 2.59 & 60  & 94  & 71  & 160 & 5.73 & 3.76 & 10.3 & 21.2 & 0.8 & 2.2 & 3.0 & 6.3  & 2.0 & 2.7 & 0.13 & 2.59 &  \\
54  & MWISP G24.421$+$0.158 & 113.98 & 1.61 & 149 & 197 & 168 & 156 & 6.92 & 3.41 & 12.8 & 21.1 & 2.8 & 3.0 & 3.2 & 1.3  & 1.7 & 1.2 & 0.14 & 1.60 &  \\
55  & MWISP G24.395$+$0.216 & 116.98 & 1.63 & 135 & 218 & 162 & 65  & 7.21 & 3.37 & 9.8  & 21.0 & 2.9 & 2.9 & 3.2 & 1.9  & 1.5 & 1.2 & 0.13 & 1.63 &  \\
56  & MWISP G24.498$-$0.217 & 97.76  & 1.72 & 97  & 196 & 123 & 8   & 5.62 & 3.83 & 11.8 & 21.1 & 1.8 & 2.7 & 3.0 & 2.4  & 1.7 & 1.7 & 0.14 & 1.71 &  \\
57  & MWISP G24.635$-$0.216 & 98.37  & 1.70 & 115 & 173 & 135 & 13  & 5.71 & 3.80 & 22.8 & 21.5 & 1.8 & 3.0 & 3.0 & 1.0  & 2.0 & 1.6 & 0.19 & 1.69 &  \\
58  & MWISP G24.865$+$0.000 & 108.42 & 2.78 & 108 & 179 & 131 & 110 & 6.14 & 3.65 & 15.5 & 21.5 & 1.9 & 3.1 & 3.5 & 2.5  & 2.0 & 2.0 & 0.16 & 2.78 &  \\
59  & MWISP G24.242$+$0.002 & 90.62  & 1.98 & 93  & 159 & 113 & 144 & 5.27 & 3.98 & 12.2 & 21.2 & 1.4 & 2.6 & 3.1 & 3.1  & 1.8 & 2.0 & 0.14 & 1.97 &  \\
60  & MWISP G24.652$-$0.216 & 112.23 & 2.91 & 147 & 253 & 180 & 77  & 6.63 & 3.49 & 23.1 & 21.7 & 3.0 & 3.7 & 3.7 & 1.1  & 2.2 & 1.7 & 0.19 & 2.90 &  \\
61  & MWISP G24.164$-$0.080 & 78.59  & 1.24 & 95  & 195 & 120 & 86  & 5.09 & 4.08 & 11.2 & 20.9 & 1.6 & 2.4 & 2.7 & 2.1  & 1.5 & 1.5 & 0.13 & 1.23 &  \\
62  & MWISP G24.398$-$0.008 & 116.02 & 2.73 & 207 & 329 & 248 & 69  & 7.21 & 3.37 & 15.8 & 21.5 & 4.5 & 3.8 & 3.8 & 1.1  & 2.0 & 1.3 & 0.16 & 2.73 &  \\
63  & MWISP G24.714$+$0.060 & 111.73 & 2.00 & 75  & 176 & 98  & 81  & 6.64 & 3.49 & 9.3  & 21.0 & 1.7 & 2.6 & 3.1 & 3.8  & 1.6 & 1.9 & 0.12 & 2.00 &  \\
64  & MWISP G24.265$+$0.167 & 112.23 & 1.89 & 134 & 154 & 143 & 34  & 7.19 & 3.36 & 11.7 & 21.1 & 2.4 & 2.9 & 3.2 & 2.0  & 1.7 & 1.5 & 0.14 & 1.88 &  \\
65  & MWISP G24.128$+$0.402 & 94.45  & 3.22 & 102 & 148 & 119 & 20  & 5.24 & 3.99 & 7.3  & 21.1 & 1.4 & 2.5 & 3.5 & 10.9 & 1.6 & 2.4 & 0.11 & 3.22 &  \\
66  & MWISP G24.336$+$0.156 & 111.11 & 2.15 & 119 & 126 & 122 & 13  & 7.19 & 3.37 & 10.1 & 21.1 & 2.0 & 2.8 & 3.3 & 3.2  & 1.7 & 1.8 & 0.13 & 2.15 &  \\
67  & MWISP G24.468$+$0.295 & 121.26 & 2.68 & 110 & 207 & 138 & 119 & 6.93 & 3.41 & 9.6  & 21.2 & 2.4 & 3.0 & 3.6 & 3.7  & 1.7 & 1.8 & 0.13 & 2.68 &  \\
68  & MWISP G24.856$+$0.020 & 104.93 & 2.04 & 102 & 204 & 129 & 63  & 6.01 & 3.70 & 15.3 & 21.3 & 2.0 & 3.0 & 3.2 & 1.8  & 1.9 & 1.7 & 0.16 & 2.03 &  \\
69  & MWISP G24.702$+$0.034 & 109.36 & 1.89 & 116 & 229 & 146 & 95  & 5.88 & 3.73 & 11.9 & 21.1 & 2.2 & 2.9 & 3.2 & 2.2  & 1.7 & 1.6 & 0.14 & 1.88 &  \\
70  & MWISP G24.272$+$0.089 & 99.84  & 2.11 & 163 & 187 & 174 & 113 & 5.71 & 3.77 & 11.0 & 21.1 & 2.3 & 2.9 & 3.3 & 2.6  & 1.7 & 1.6 & 0.13 & 2.11 &  \\
71  & MWISP G24.435$+$0.101 & 114.32 & 1.94 & 207 & 499 & 270 & 145 & 6.98 & 3.40 & 15.7 & 21.3 & 5.4 & 3.8 & 3.6 & 0.7  & 1.8 & 0.8 & 0.16 & 1.93 &  \\
72  & MWISP G24.190$-$0.146 & 79.56  & 1.50 & 150 & 201 & 170 & 46  & 5.07 & 4.09 & 8.3  & 20.8 & 2.0 & 2.5 & 3.0 & 3.2  & 1.4 & 1.4 & 0.12 & 1.50 &  \\
73  & MWISP G24.448$+$0.217 & 121.62 & 2.13 & 210 & 231 & 220 & 52  & 7.16 & 3.38 & 9.8  & 21.1 & 3.7 & 3.3 & 3.5 & 2.0  & 1.6 & 1.2 & 0.13 & 2.13 &  \\
74  & MWISP G24.392$+$0.175 & 110.32 & 1.46 & 107 & 175 & 129 & 17  & 6.21 & 3.58 & 12.0 & 21.0 & 1.9 & 2.7 & 2.9 & 1.8  & 1.6 & 1.5 & 0.14 & 1.45 &  \\
75  & MWISP G24.501$+$0.467 & 102.06 & 0.83 & 58  & 79  & 66  & 146 & 5.47 & 3.90 & 11.9 & 20.8 & 0.6 & 1.7 & 1.9 & 1.8  & 1.6 & 2.0 & 0.14 & 0.82 &  \\
76  & MWISP G24.682$-$0.069 & 90.95  & 4.25 & 190 & 232 & 208 & 40  & 5.40 & 3.95 & 12.1 & 21.5 & 2.7 & 3.4 & 4.0 & 4.1  & 2.0 & 2.1 & 0.14 & 4.25 &  \\
77  & MWISP G24.701$-$0.119 & 107.30 & 4.18 & 123 & 172 & 141 & 100 & 5.47 & 3.92 & 15.8 & 21.7 & 1.8 & 3.2 & 3.8 & 3.9  & 2.2 & 2.4 & 0.16 & 4.18 &  \\
78  & MWISP G24.430$+$0.357 & 113.80 & 1.77 & 133 & 268 & 169 & 113 & 6.60 & 3.47 & 10.2 & 21.0 & 2.9 & 3.0 & 3.3 & 1.9  & 1.6 & 1.3 & 0.13 & 1.77 &  \\
79  & MWISP G24.734$+$0.147 & 106.84 & 1.32 & 81  & 134 & 98  & 127 & 6.04 & 3.67 & 18.4 & 21.2 & 1.4 & 2.6 & 2.7 & 1.2  & 1.9 & 1.7 & 0.17 & 1.31 &  \\
80  & MWISP G24.417$-$0.258 & 96.65  & 1.64 & 63  & 127 & 80  & -23 & 5.49 & 3.88 & 12.4 & 21.1 & 1.0 & 2.3 & 2.7 & 3.0  & 1.8 & 2.1 & 0.14 & 1.63 &  \\
81  & MWISP G24.804$+$0.112 & 111.24 & 1.48 & 74  & 137 & 92  & 112 & 6.49 & 3.54 & 16.8 & 21.2 & 1.4 & 2.6 & 2.8 & 1.4  & 1.9 & 1.8 & 0.17 & 1.47 &  \\
82  & MWISP G24.232$-$0.051 & 89.36  & 1.68 & 142 & 318 & 184 & -2  & 5.22 & 4.01 & 10.4 & 21.0 & 2.6 & 2.9 & 3.2 & 2.0  & 1.6 & 1.3 & 0.13 & 1.67 &  \\
83  & MWISP G24.545$-$0.244 & 97.13  & 1.69 & 96  & 112 & 103 & 56  & 5.59 & 3.85 & 12.9 & 21.1 & 1.2 & 2.4 & 2.9 & 2.6  & 1.8 & 2.0 & 0.15 & 1.68 &  \\
84  & MWISP G24.130$+$0.020 & 97.14  & 1.84 & 78  & 95  & 85  & -25 & 5.50 & 3.85 & 14.1 & 21.2 & 0.9 & 2.4 & 2.8 & 2.9  & 1.9 & 2.3 & 0.15 & 1.83 &  \\
85  & MWISP G24.622$-$0.185 & 96.67  & 1.93 & 145 & 233 & 174 & -20 & 5.64 & 3.83 & 9.8  & 21.0 & 2.4 & 2.8 & 3.3 & 2.7  & 1.6 & 1.5 & 0.13 & 1.93 &  \\
86  & MWISP G24.517$+$0.508 & 101.91 & 1.26 & 73  & 184 & 96  & 25  & 5.64 & 3.82 & 10.6 & 20.9 & 1.4 & 2.3 & 2.7 & 2.3  & 1.5 & 1.6 & 0.13 & 1.25 &  \\
87  & MWISP G24.417$+$0.083 & 111.13 & 1.58 & 94  & 253 & 125 & 109 & 6.76 & 3.43 & 20.2 & 21.4 & 2.4 & 3.2 & 3.1 & 0.8  & 1.9 & 1.3 & 0.18 & 1.57 &  \\
88  & MWISP G24.710$-$0.265 & 94.76  & 3.35 & 269 & 327 & 294 & 48  & 5.51 & 3.90 & 17.5 & 21.6 & 3.9 & 3.8 & 4.0 & 1.4  & 2.1 & 1.6 & 0.17 & 3.35 &  \\
89  & MWISP G24.655$-$0.366 & 112.56 & 2.03 & 116 & 305 & 153 & 146 & 6.42 & 3.54 & 7.9  & 20.9 & 2.8 & 2.9 & 3.4 & 3.4  & 1.5 & 1.4 & 0.11 & 2.03 &  \\
90  & MWISP G24.890$+$0.477 & 108.42 & 2.06 & 80  & 154 & 101 & -3  & 5.91 & 3.74 & 12.3 & 21.2 & 1.4 & 2.6 & 3.1 & 3.1  & 1.8 & 2.0 & 0.14 & 2.06 &  \\
91  & MWISP G24.274$+$0.159 & 114.13 & 1.34 & 142 & 216 & 168 & -6  & 7.23 & 3.36 & 10.6 & 20.9 & 3.0 & 2.9 & 3.0 & 1.4  & 1.5 & 1.0 & 0.13 & 1.33 &  \\
92  & MWISP G24.670$-$0.162 & 115.55 & 2.38 & 92  & 149 & 111 & 136 & 6.95 & 3.43 & 14.2 & 21.4 & 1.8 & 2.9 & 3.3 & 2.4  & 1.9 & 1.9 & 0.15 & 2.38 &  \\
93  & MWISP G24.117$+$0.252 & 112.08 & 1.21 & 78  & 196 & 102 & 172 & 7.25 & 3.34 & 10.3 & 20.9 & 2.0 & 2.5 & 2.8 & 1.7  & 1.5 & 1.3 & 0.13 & 1.20 &  \\
94  & MWISP G24.243$+$0.212 & 112.69 & 1.33 & 155 & 229 & 182 & 42  & 7.23 & 3.35 & 11.9 & 21.0 & 3.2 & 3.0 & 3.1 & 1.1  & 1.5 & 0.9 & 0.14 & 1.32 &  \\
95  & MWISP G24.137$+$0.208 & 114.73 & 1.60 & 120 & 184 & 142 & 2   & 7.60 & 3.34 & 12.3 & 21.1 & 2.6 & 3.0 & 3.1 & 1.5  & 1.7 & 1.3 & 0.14 & 1.59 &  \\
96  & MWISP G24.393$+$0.194 & 114.77 & 1.16 & 126 & 202 & 151 & 27  & 7.18 & 3.37 & 10.1 & 20.8 & 2.6 & 2.7 & 2.9 & 1.4  & 1.4 & 1.0 & 0.13 & 1.15 &  \\
97  & MWISP G24.158$+$0.169 & 107.48 & 1.18 & 115 & 185 & 138 & -10 & 6.18 & 3.56 & 12.4 & 21.0 & 2.1 & 2.7 & 2.8 & 1.3  & 1.5 & 1.2 & 0.14 & 1.17 &  \\
98  & MWISP G24.542$+$0.503 & 109.37 & 2.06 & 107 & 128 & 116 & 113 & 6.03 & 3.66 & 8.5  & 21.0 & 1.6 & 2.4 & 3.1 & 5.0  & 1.6 & 1.9 & 0.12 & 2.06 &  \\
99  & MWISP G24.396$+$0.024 & 110.64 & 2.05 & 62  & 124 & 78  & 28  & 6.76 & 3.43 & 17.6 & 21.4 & 1.2 & 2.7 & 3.0 & 2.0  & 2.1 & 2.2 & 0.17 & 2.04 &  \\
100 & MWISP G24.418$+$0.357 & 110.96 & 1.93 & 89  & 130 & 104 & 120 & 6.79 & 3.43 & 7.2  & 20.8 & 1.6 & 2.3 & 3.1 & 5.7  & 1.4 & 1.9 & 0.11 & 1.93 &  \\
101 & MWISP G24.729$+$0.154 & 110.15 & 2.16 & 68  & 82  & 74  & -64 & 6.39 & 3.56 & 16.3 & 21.4 & 0.9 & 2.5 & 2.9 & 2.6  & 2.1 & 2.5 & 0.16 & 2.15 &  \\
102 & MWISP G24.536$+$0.484 & 103.48 & 1.60 & 154 & 269 & 189 & 111 & 5.68 & 3.80 & 12.0 & 21.1 & 2.7 & 3.0 & 3.2 & 1.5  & 1.6 & 1.2 & 0.14 & 1.59 &  \\
103 & MWISP G24.369$+$0.110 & 112.70 & 1.78 & 147 & 384 & 194 & 107 & 6.91 & 3.40 & 17.0 & 21.3 & 3.9 & 3.5 & 3.4 & 0.8  & 1.9 & 1.0 & 0.17 & 1.77 &  \\
104 & MWISP G24.342$+$0.284 & 110.16 & 0.93 & 73  & 87  & 79  & 108 & 6.30 & 3.54 & 11.7 & 20.8 & 1.0 & 2.0 & 2.2 & 1.7  & 1.5 & 1.7 & 0.14 & 0.92 &  \\
105 & MWISP G24.375$+$0.306 & 110.79 & 1.42 & 85  & 153 & 105 & 117 & 6.92 & 3.40 & 11.2 & 21.0 & 1.7 & 2.6 & 2.9 & 2.0  & 1.6 & 1.5 & 0.13 & 1.41 &  \\
106 & MWISP G24.211$-$0.315 & 88.59  & 2.43 & 112 & 205 & 139 & 111 & 5.05 & 4.10 & 5.7  & 20.7 & 1.8 & 2.3 & 3.3 & 11.3 & 1.3 & 2.0 & 0.10 & 2.43 &  \\
107 & MWISP G24.776$-$0.027 & 108.74 & 2.40 & 128 & 291 & 166 & 41  & 5.33 & 3.99 & 15.4 & 21.4 & 2.4 & 3.2 & 3.5 & 1.8  & 1.9 & 1.7 & 0.16 & 2.39 &  \\
108 & MWISP G24.518$+$0.264 & 110.95 & 2.60 & 184 & 207 & 194 & 88  & 5.97 & 3.68 & 8.3  & 21.1 & 2.7 & 3.0 & 3.6 & 4.2  & 1.6 & 1.7 & 0.12 & 2.60 &  \\
109 & MWISP G24.434$-$0.214 & 97.47  & 1.82 & 122 & 145 & 132 & 22  & 5.58 & 3.84 & 14.4 & 21.2 & 1.7 & 2.8 & 3.1 & 2.0  & 1.8 & 1.8 & 0.15 & 1.81 &  \\
110 & MWISP G24.408$-$0.017 & 112.87 & 1.52 & 173 & 217 & 192 & 84  & 6.95 & 3.40 & 15.2 & 21.2 & 3.2 & 3.2 & 3.2 & 0.9  & 1.7 & 1.1 & 0.16 & 1.51 &  \\
111 & MWISP G24.275$-$0.024 & 85.87  & 1.99 & 80  & 93  & 86  & 44  & 5.18 & 4.04 & 9.2  & 21.0 & 0.9 & 2.1 & 2.9 & 6.0  & 1.7 & 2.4 & 0.12 & 1.99 &  \\
112 & MWISP G24.449$-$0.338 & 97.14  & 1.78 & 97  & 227 & 126 & 114 & 5.46 & 3.90 & 11.1 & 21.1 & 1.9 & 2.7 & 3.1 & 2.6  & 1.6 & 1.7 & 0.13 & 1.77 &  \\
113 & MWISP G24.335$+$0.106 & 101.75 & 2.16 & 73  & 105 & 85  & 50  & 5.82 & 3.72 & 11.3 & 21.2 & 1.0 & 2.4 & 3.0 & 4.3  & 1.8 & 2.4 & 0.14 & 2.16 &  \\
114 & MWISP G24.815$+$0.047 & 104.45 & 2.24 & 146 & 176 & 159 & 77  & 5.99 & 3.70 & 18.5 & 21.5 & 2.2 & 3.2 & 3.4 & 1.4  & 2.0 & 1.7 & 0.17 & 2.23 &  \\
115 & MWISP G24.476$+$0.276 & 118.88 & 1.84 & 63  & 144 & 82  & 121 & 6.97 & 3.41 & 9.5  & 21.0 & 1.4 & 2.4 & 3.0 & 3.7  & 1.6 & 1.9 & 0.12 & 1.84 &  \\
116 & MWISP G24.581$-$0.258 & 97.31  & 1.86 & 78  & 127 & 95  & 21  & 5.61 & 3.84 & 10.1 & 21.0 & 1.2 & 2.3 & 2.9 & 4.1  & 1.7 & 2.1 & 0.13 & 1.86 &  \\
117 & MWISP G24.424$+$0.312 & 104.77 & 1.67 & 91  & 268 & 122 & 14  & 5.75 & 3.76 & 9.7  & 21.0 & 2.1 & 2.7 & 3.1 & 2.7  & 1.5 & 1.5 & 0.13 & 1.67 &  \\
118 & MWISP G24.451$+$0.506 & 102.85 & 0.99 & 72  & 184 & 95  & 145 & 5.65 & 3.81 & 13.9 & 21.0 & 1.4 & 2.4 & 2.5 & 1.3  & 1.6 & 1.4 & 0.15 & 0.98 &  \\
119 & MWISP G24.128$+$0.117 & 112.38 & 1.48 & 56  & 81  & 65  & -9  & 7.39 & 3.33 & 11.7 & 21.0 & 0.8 & 2.2 & 2.6 & 2.4  & 1.9 & 2.2 & 0.14 & 1.47 &  \\
120 & MWISP G24.786$+$0.073 & 109.36 & 1.60 & 64  & 156 & 84  & 121 & 6.32 & 3.58 & 20.3 & 21.4 & 1.3 & 2.7 & 2.9 & 1.3  & 2.0 & 1.9 & 0.18 & 1.59 &  \\
121 & MWISP G24.174$-$0.077 & 89.99  & 2.08 & 89  & 197 & 114 & 142 & 5.21 & 4.01 & 11.1 & 21.1 & 1.5 & 2.6 & 3.1 & 3.5  & 1.7 & 2.0 & 0.13 & 2.08 &  \\
122 & MWISP G24.515$+$0.466 & 101.62 & 0.86 & 130 & 363 & 173 & 135 & 5.63 & 3.82 & 13.3 & 20.9 & 2.9 & 2.8 & 2.7 & 0.7  & 1.4 & 0.6 & 0.15 & 0.85 &  \\
123 & MWISP G24.812$+$0.127 & 109.52 & 2.42 & 70  & 135 & 88  & 137 & 6.28 & 3.60 & 17.8 & 21.5 & 1.3 & 2.8 & 3.2 & 2.3  & 2.1 & 2.3 & 0.17 & 2.41 &  \\
124 & MWISP G24.526$-$0.191 & 99.53  & 1.63 & 71  & 94  & 80  & -8  & 5.73 & 3.78 & 19.6 & 21.4 & 0.9 & 2.5 & 2.7 & 1.7  & 2.1 & 2.2 & 0.18 & 1.62 &  \\
125 & MWISP G25.028$+$0.047 & 106.97 & 1.30 & 142 & 215 & 167 & -5  & 6.08 & 3.69 & 14.8 & 21.1 & 2.5 & 2.9 & 2.9 & 1.0  & 1.7 & 1.1 & 0.16 & 1.29 &  \\
126 & MWISP G24.655$-$0.306 & 114.44 & 3.07 & 149 & 275 & 185 & 111 & 6.88 & 3.44 & 13.2 & 21.4 & 3.3 & 3.5 & 3.8 & 2.1  & 2.0 & 1.6 & 0.15 & 3.07 &  \\
127 & MWISP G24.324$-$0.001 & 115.72 & 1.99 & 178 & 187 & 182 & -56 & 7.29 & 3.36 & 18.0 & 21.4 & 3.1 & 3.4 & 3.4 & 1.0  & 1.9 & 1.3 & 0.17 & 1.98 &  \\
128 & MWISP G24.372$+$0.309 & 113.49 & 1.43 & 101 & 186 & 125 & 95  & 6.65 & 3.45 & 11.1 & 21.0 & 2.1 & 2.7 & 2.9 & 1.9  & 1.6 & 1.4 & 0.13 & 1.42 &  \\
129 & MWISP G24.612$-$0.112 & 83.64  & 3.06 & 165 & 260 & 197 & 121 & 5.21 & 4.04 & 12.2 & 21.4 & 2.5 & 3.2 & 3.7 & 3.1  & 1.9 & 1.9 & 0.14 & 3.06 &  \\
130 & MWISP G24.770$-$0.224 & 78.89  & 2.35 & 197 & 380 & 247 & 19  & 5.17 & 4.08 & 15.0 & 21.4 & 3.4 & 3.5 & 3.6 & 1.4  & 1.9 & 1.4 & 0.16 & 2.34 &  \\
131 & MWISP G24.765$+$0.138 & 109.06 & 1.83 & 123 & 216 & 151 & 94  & 6.25 & 3.60 & 20.0 & 21.4 & 2.4 & 3.2 & 3.2 & 1.0  & 2.0 & 1.5 & 0.18 & 1.82 &  \\
132 & MWISP G24.598$+$0.444 & 108.11 & 1.84 & 72  & 203 & 96  & 76  & 5.93 & 3.70 & 14.5 & 21.3 & 1.6 & 2.7 & 3.0 & 2.1  & 1.8 & 1.8 & 0.15 & 1.83 &  \\
133 & MWISP G25.069$-$0.025 & 102.07 & 2.46 & 95  & 118 & 105 & 137 & 5.92 & 3.75 & 13.1 & 21.3 & 1.4 & 2.7 & 3.2 & 3.5  & 1.9 & 2.2 & 0.15 & 2.46 &  \\
134 & MWISP G24.434$+$0.015 & 111.60 & 1.98 & 144 & 190 & 163 & 26  & 6.82 & 3.42 & 15.4 & 21.3 & 2.6 & 3.2 & 3.3 & 1.4  & 1.9 & 1.5 & 0.16 & 1.97 &  \\
135 & MWISP G24.402$+$0.179 & 115.87 & 1.25 & 92  & 133 & 107 & 174 & 7.21 & 3.37 & 11.2 & 20.9 & 1.7 & 2.5 & 2.8 & 1.8  & 1.5 & 1.4 & 0.13 & 1.24 &  \\
136 & MWISP G24.399$+$0.277 & 109.99 & 1.15 & 140 & 328 & 182 & 121 & 6.63 & 3.46 & 10.1 & 20.8 & 3.4 & 2.9 & 3.0 & 1.1  & 1.4 & 0.8 & 0.13 & 1.14 &  \\
137 & MWISP G24.814$+$0.031 & 108.42 & 1.62 & 79  & 209 & 105 & -3  & 5.50 & 3.91 & 18.0 & 21.3 & 1.6 & 2.8 & 2.9 & 1.4  & 1.9 & 1.7 & 0.17 & 1.61 &  \\
138 & MWISP G24.164$+$0.000 & 78.24  & 1.27 & 82  & 193 & 107 & 17  & 5.11 & 4.07 & 13.2 & 21.0 & 1.4 & 2.4 & 2.7 & 1.8  & 1.6 & 1.6 & 0.15 & 1.26 &  \\
139 & MWISP G24.259$+$0.056 & 112.68 & 2.76 & 234 & 409 & 287 & 12  & 7.24 & 3.35 & 12.2 & 21.3 & 5.4 & 3.8 & 3.9 & 1.3  & 1.8 & 1.1 & 0.14 & 2.76 &  \\
140 & MWISP G24.825$-$0.147 & 89.55  & 1.77 & 186 & 235 & 207 & 158 & 5.34 & 3.99 & 11.8 & 21.1 & 2.6 & 3.0 & 3.2 & 1.8  & 1.6 & 1.4 & 0.14 & 1.76 &  \\
141 & MWISP G24.351$+$0.210 & 115.40 & 1.04 & 70  & 120 & 86  & 150 & 7.20 & 3.37 & 10.5 & 20.8 & 1.4 & 2.2 & 2.5 & 1.8  & 1.5 & 1.5 & 0.13 & 1.03 &  \\
142 & MWISP G24.478$+$0.325 & 110.15 & 2.09 & 223 & 291 & 250 & 123 & 7.00 & 3.40 & 9.1  & 21.0 & 4.2 & 3.3 & 3.6 & 1.9  & 1.6 & 1.1 & 0.12 & 2.09 &  \\
143 & MWISP G24.713$+$0.100 & 108.42 & 2.09 & 114 & 143 & 126 & 90  & 5.32 & 3.99 & 15.3 & 21.3 & 1.5 & 2.8 & 3.1 & 2.3  & 1.9 & 2.0 & 0.16 & 2.08 &  \\
144 & MWISP G24.267$+$0.259 & 113.17 & 1.56 & 103 & 156 & 122 & -12 & 6.70 & 3.43 & 10.6 & 21.0 & 1.9 & 2.6 & 3.0 & 2.3  & 1.6 & 1.5 & 0.13 & 1.55 &  \\
145 & MWISP G24.553$+$0.226 & 118.41 & 2.79 & 88  & 178 & 112 & 102 & 7.16 & 3.40 & 13.4 & 21.4 & 2.0 & 3.1 & 3.5 & 2.8  & 2.0 & 2.0 & 0.15 & 2.79 &  \\
146 & MWISP G24.435$+$0.145 & 111.27 & 2.44 & 216 & 333 & 256 & 37  & 6.72 & 3.44 & 14.1 & 21.4 & 4.3 & 3.6 & 3.7 & 1.2  & 1.9 & 1.2 & 0.15 & 2.44 &  \\
147 & MWISP G24.333$+$0.291 & 111.27 & 1.21 & 79  & 130 & 95  & 128 & 7.00 & 3.39 & 12.4 & 21.0 & 1.5 & 2.5 & 2.7 & 1.6  & 1.6 & 1.5 & 0.14 & 1.20 &  \\
148 & MWISP G24.167$+$0.249 & 112.39 & 1.32 & 88  & 158 & 109 & 154 & 7.21 & 3.34 & 11.2 & 21.0 & 1.9 & 2.6 & 2.8 & 1.8  & 1.5 & 1.4 & 0.13 & 1.31 &  \\
149 & MWISP G24.459$+$0.435 & 104.28 & 1.27 & 93  & 220 & 121 & 26  & 5.67 & 3.80 & 7.0  & 20.6 & 1.9 & 2.2 & 2.8 & 3.8  & 1.2 & 1.4 & 0.11 & 1.27 &  \\
150 & MWISP G24.802$-$0.104 & 80.48  & 2.23 & 153 & 286 & 191 & 70  & 5.26 & 4.03 & 10.4 & 21.1 & 2.6 & 3.0 & 3.4 & 2.7  & 1.7 & 1.6 & 0.13 & 2.23 &  \\
151 & MWISP G24.523$+$0.335 & 104.13 & 1.93 & 119 & 208 & 146 & 139 & 5.78 & 3.76 & 8.6  & 21.0 & 2.1 & 2.6 & 3.2 & 3.7  & 1.5 & 1.6 & 0.12 & 1.93 &  \\
152 & MWISP G24.447$+$0.383 & 115.72 & 1.70 & 154 & 252 & 186 & 103 & 6.65 & 3.46 & 9.6  & 21.0 & 3.1 & 3.0 & 3.3 & 1.9  & 1.5 & 1.2 & 0.13 & 1.70 &  \\
153 & MWISP G24.168$-$0.017 & 100.15 & 1.82 & 65  & 71  & 67  & 8   & 5.67 & 3.78 & 13.5 & 21.2 & 0.6 & 2.1 & 2.6 & 3.2  & 2.0 & 2.6 & 0.15 & 1.81 &  \\
154 & MWISP G24.515$+$0.268 & 118.09 & 1.60 & 85  & 105 & 93  & 145 & 7.14 & 3.39 & 8.0  & 20.8 & 1.4 & 2.3 & 2.9 & 4.2  & 1.5 & 1.8 & 0.11 & 1.60 &  \\
155 & MWISP G24.419$+$0.305 & 106.35 & 1.31 & 86  & 206 & 112 & 14  & 6.67 & 3.45 & 10.9 & 20.9 & 2.0 & 2.6 & 2.9 & 1.8  & 1.5 & 1.3 & 0.13 & 1.30 &  \\
156 & MWISP G24.507$+$0.444 & 102.53 & 0.82 & 125 & 176 & 144 & 147 & 5.65 & 3.81 & 13.4 & 20.9 & 1.9 & 2.5 & 2.4 & 0.9  & 1.4 & 1.0 & 0.15 & 0.81 &  \\
157 & MWISP G24.413$+$0.293 & 108.89 & 0.96 & 88  & 210 & 115 & 107 & 6.88 & 3.41 & 11.6 & 20.8 & 2.1 & 2.6 & 2.6 & 1.1  & 1.4 & 1.0 & 0.14 & 0.95 &  \\
158 & MWISP G24.655$-$0.184 & 108.58 & 2.45 & 95  & 141 & 111 & 87  & 6.24 & 3.59 & 10.1 & 21.2 & 1.6 & 2.7 & 3.3 & 4.4  & 1.8 & 2.1 & 0.13 & 2.45 &  \\
159 & MWISP G24.373$+$0.318 & 112.21 & 1.24 & 139 & 329 & 181 & 126 & 6.99 & 3.39 & 10.2 & 20.9 & 3.5 & 3.0 & 3.1 & 1.1  & 1.4 & 0.8 & 0.13 & 1.23 &  \\
160 & MWISP G24.293$+$0.266 & 111.12 & 1.03 & 71  & 172 & 93  & 15  & 7.05 & 3.37 & 11.5 & 20.9 & 1.7 & 2.4 & 2.6 & 1.4  & 1.5 & 1.3 & 0.14 & 1.02 &  \\
161 & MWISP G24.449$+$0.483 & 101.75 & 0.47 & 56  & 151 & 74  & 69  & 5.62 & 3.82 & 12.8 & 20.6 & 1.1 & 1.8 & 1.7 & 0.8  & 1.2 & 1.0 & 0.14 & 0.45 &  \\
162 & MWISP G24.401$+$0.249 & 117.78 & 1.09 & 76  & 97  & 85  & 149 & 7.19 & 3.37 & 9.4  & 20.8 & 1.2 & 2.1 & 2.5 & 2.3  & 1.4 & 1.6 & 0.12 & 1.08 &  \\
163 & MWISP G24.637$-$0.258 & 97.13  & 1.32 & 103 & 171 & 124 & -12 & 5.62 & 3.84 & 23.8 & 21.4 & 1.7 & 2.9 & 2.8 & 0.8  & 1.9 & 1.5 & 0.20 & 1.31 &  \\
164 & MWISP G24.385$+$0.139 & 114.78 & 2.66 & 275 & 447 & 331 & 130 & 7.18 & 3.37 & 15.2 & 21.4 & 6.0 & 4.0 & 4.0 & 0.9  & 2.0 & 1.0 & 0.16 & 2.66 &  \\
165 & MWISP G24.497$-$0.282 & 96.98  & 1.82 & 86  & 102 & 93  & -17 & 5.53 & 3.87 & 15.4 & 21.3 & 1.1 & 2.5 & 2.9 & 2.4  & 1.9 & 2.2 & 0.16 & 1.81 &  \\
166 & MWISP G24.476$+$0.506 & 102.38 & 1.17 & 54  & 91  & 66  & 14  & 5.65 & 3.81 & 13.4 & 21.0 & 0.7 & 2.0 & 2.3 & 2.1  & 1.8 & 2.2 & 0.15 & 1.16 &  \\
167 & MWISP G24.936$+$0.139 & 91.73  & 1.11 & 87  & 129 & 102 & 78  & 5.57 & 3.89 & 14.1 & 21.0 & 1.3 & 2.3 & 2.5 & 1.5  & 1.6 & 1.6 & 0.15 & 1.10 &  \\
168 & MWISP G24.423$+$0.221 & 118.25 & 1.42 & 93  & 237 & 123 & 107 & 7.21 & 3.38 & 10.6 & 21.0 & 2.4 & 2.8 & 3.0 & 1.7  & 1.5 & 1.2 & 0.13 & 1.41 &  \\
169 & MWISP G24.423$+$0.473 & 103.78 & 0.96 & 116 & 172 & 136 & 127 & 5.66 & 3.80 & 12.7 & 20.9 & 1.8 & 2.5 & 2.5 & 1.2  & 1.5 & 1.1 & 0.14 & 0.95 &  \\
170 & MWISP G24.539$+$0.301 & 107.92 & 1.03 & 101 & 191 & 127 & 61  & 6.61 & 3.48 & 10.2 & 20.8 & 2.1 & 2.5 & 2.7 & 1.5  & 1.4 & 1.1 & 0.13 & 1.02 &  \\
171 & MWISP G24.258$+$0.068 & 98.23  & 1.49 & 88  & 216 & 116 & 141 & 5.62 & 3.81 & 13.0 & 21.1 & 1.8 & 2.7 & 2.9 & 1.8  & 1.7 & 1.6 & 0.15 & 1.48 &  \\
172 & MWISP G24.270$+$0.444 & 96.20  & 3.26 & 163 & 191 & 175 & 89  & 5.36 & 3.94 & 8.2  & 21.1 & 2.2 & 2.9 & 3.7 & 6.6  & 1.7 & 2.0 & 0.12 & 3.26 &  \\
173 & MWISP G24.432$-$0.315 & 95.55  & 2.10 & 102 & 137 & 115 & 150 & 5.38 & 3.94 & 14.0 & 21.3 & 1.4 & 2.7 & 3.1 & 2.8  & 1.9 & 2.1 & 0.15 & 2.09 &  \\
174 & MWISP G24.342$-$0.301 & 98.72  & 2.01 & 78  & 157 & 99  & 6   & 5.52 & 3.86 & 9.7  & 21.1 & 1.3 & 2.4 & 3.1 & 4.5  & 1.7 & 2.1 & 0.13 & 2.01 &  \\
175 & MWISP G24.273$-$0.085 & 89.21  & 2.40 & 81  & 169 & 103 & 94  & 5.22 & 4.01 & 9.9  & 21.1 & 1.3 & 2.5 & 3.2 & 5.3  & 1.7 & 2.2 & 0.13 & 2.40 &  \\
176 & MWISP G24.334$+$0.234 & 113.65 & 0.72 & 90  & 159 & 110 & 68  & 7.13 & 3.37 & 11.5 & 20.7 & 1.9 & 2.3 & 2.3 & 0.9  & 1.3 & 0.9 & 0.14 & 0.71 &  \\
177 & MWISP G24.177$+$0.049 & 109.05 & 2.97 & 193 & 346 & 238 & 4   & 5.60 & 3.81 & 15.1 & 21.5 & 3.4 & 3.6 & 3.8 & 1.7  & 2.0 & 1.6 & 0.16 & 2.97 &  \\
178 & MWISP G24.960$+$0.051 & 105.88 & 0.91 & 64  & 126 & 80  & 47  & 6.04 & 3.69 & 13.7 & 20.9 & 1.1 & 2.2 & 2.3 & 1.3  & 1.6 & 1.5 & 0.15 & 0.90 &  \\
179 & MWISP G24.420$-$0.049 & 110.16 & 2.08 & 109 & 233 & 139 & 95  & 7.45 & 3.37 & 13.5 & 21.3 & 2.7 & 3.2 & 3.4 & 1.6  & 1.8 & 1.5 & 0.15 & 2.07 &  \\
180 & MWISP G24.536$+$0.331 & 106.67 & 1.61 & 193 & 249 & 216 & 84  & 5.98 & 3.68 & 8.9  & 20.9 & 3.1 & 2.9 & 3.2 & 2.1  & 1.4 & 1.1 & 0.12 & 1.61 &  \\
181 & MWISP G24.622$-$0.172 & 80.00  & 3.62 & 279 & 412 & 326 & 29  & 5.17 & 4.07 & 11.1 & 21.4 & 4.2 & 3.6 & 4.1 & 2.6  & 1.9 & 1.6 & 0.13 & 3.62 &  \\
182 & MWISP G24.618$-$0.418 & 113.50 & 2.34 & 136 & 247 & 168 & 92  & 6.48 & 3.52 & 7.3  & 20.9 & 2.8 & 2.8 & 3.5 & 4.5  & 1.5 & 1.6 & 0.11 & 2.34 &  \\
183 & MWISP G24.627$-$0.169 & 114.11 & 1.87 & 101 & 178 & 124 & 65  & 6.86 & 3.44 & 11.1 & 21.1 & 2.1 & 2.8 & 3.2 & 2.4  & 1.7 & 1.6 & 0.13 & 1.87 &  \\
184 & MWISP G24.585$-$0.211 & 99.21  & 1.73 & 96  & 118 & 105 & 6   & 5.73 & 3.78 & 13.9 & 21.2 & 1.3 & 2.5 & 2.9 & 2.3  & 1.8 & 1.9 & 0.15 & 1.72 &  \\
185 & MWISP G24.342$+$0.250 & 110.48 & 1.32 & 77  & 193 & 101 & 120 & 7.10 & 3.38 & 11.1 & 21.0 & 1.9 & 2.6 & 2.8 & 1.8  & 1.5 & 1.4 & 0.13 & 1.31 &  \\
186 & MWISP G24.441$+$0.392 & 111.91 & 1.08 & 99  & 185 & 123 & 101 & 7.21 & 3.38 & 9.3  & 20.8 & 2.2 & 2.5 & 2.7 & 1.7  & 1.3 & 1.1 & 0.12 & 1.07 &  \\
187 & MWISP G24.324$+$0.330 & 110.46 & 1.21 & 120 & 181 & 142 & 97  & 6.86 & 3.40 & 10.7 & 20.9 & 2.3 & 2.7 & 2.9 & 1.5  & 1.5 & 1.1 & 0.13 & 1.20 &  \\
188 & MWISP G24.406$+$0.506 & 108.25 & 2.13 & 118 & 137 & 126 & 105 & 5.99 & 3.66 & 9.0  & 21.0 & 1.7 & 2.6 & 3.2 & 4.4  & 1.6 & 1.9 & 0.12 & 2.13 &  \\
189 & MWISP G24.587$-$0.115 & 97.30  & 2.52 & 94  & 108 & 100 & -16 & 5.70 & 3.80 & 15.0 & 21.4 & 1.2 & 2.7 & 3.2 & 3.2  & 2.0 & 2.3 & 0.16 & 2.52 &  \\
190 & MWISP G24.242$+$0.159 & 113.17 & 0.90 & 67  & 162 & 88  & 4   & 7.18 & 3.36 & 12.2 & 20.8 & 1.6 & 2.4 & 2.4 & 1.2  & 1.5 & 1.2 & 0.14 & 0.89 &  \\
191 & MWISP G24.468$-$0.251 & 96.83  & 2.03 & 72  & 135 & 90  & 13  & 5.53 & 3.87 & 14.6 & 21.3 & 1.1 & 2.5 & 3.0 & 2.8  & 1.9 & 2.2 & 0.15 & 2.02 &  \\
192 & MWISP G24.407$+$0.498 & 102.54 & 1.46 & 57  & 78  & 65  & 4   & 5.64 & 3.81 & 11.0 & 21.0 & 0.6 & 1.9 & 2.4 & 3.4  & 1.8 & 2.5 & 0.13 & 1.45 &  \\
193 & MWISP G24.300$+$0.209 & 114.29 & 1.27 & 84  & 182 & 108 & 55  & 7.20 & 3.36 & 12.0 & 21.0 & 2.0 & 2.7 & 2.8 & 1.5  & 1.6 & 1.3 & 0.14 & 1.26 &  \\
194 & MWISP G24.752$+$0.119 & 110.79 & 2.15 & 161 & 232 & 187 & -25 & 6.48 & 3.53 & 17.3 & 21.4 & 2.9 & 3.4 & 3.5 & 1.2  & 2.0 & 1.4 & 0.17 & 2.14 &  \\
195 & MWISP G24.368$+$0.319 & 115.39 & 1.28 & 108 & 136 & 120 & 44  & 6.77 & 3.43 & 10.4 & 20.9 & 1.8 & 2.5 & 2.8 & 2.0  & 1.5 & 1.4 & 0.13 & 1.27 &  \\
196 & MWISP G24.450$+$0.434 & 102.38 & 0.87 & 97  & 250 & 128 & 48  & 5.62 & 3.82 & 6.4  & 20.4 & 2.0 & 2.0 & 2.5 & 2.9  & 0.9 & 1.0 & 0.10 & 0.86 &  \\
197 & MWISP G25.059$+$0.014 & 105.56 & 1.12 & 121 & 300 & 158 & -5  & 6.03 & 3.71 & 16.0 & 21.1 & 2.7 & 3.0 & 2.8 & 0.7  & 1.6 & 0.9 & 0.16 & 1.11 &  \\
198 & MWISP G24.645$+$0.465 & 110.16 & 2.16 & 117 & 182 & 139 & -20 & 5.85 & 3.74 & 16.0 & 21.4 & 1.9 & 3.0 & 3.3 & 1.8  & 1.9 & 1.8 & 0.16 & 2.15 &  \\
199 & MWISP G24.237$+$0.226 & 115.10 & 1.06 & 110 & 199 & 136 & 155 & 7.23 & 3.35 & 10.4 & 20.8 & 2.4 & 2.7 & 2.8 & 1.3  & 1.4 & 1.0 & 0.13 & 1.05 &  \\
200 & MWISP G24.383$+$0.250 & 114.29 & 1.09 & 74  & 159 & 95  & 112 & 7.12 & 3.38 & 9.1  & 20.7 & 1.7 & 2.3 & 2.6 & 2.1  & 1.3 & 1.3 & 0.12 & 1.08 &  \\
201 & MWISP G24.300$+$0.267 & 111.91 & 0.69 & 69  & 114 & 84  & 79  & 7.08 & 3.37 & 11.6 & 20.7 & 1.3 & 2.1 & 2.1 & 1.1  & 1.4 & 1.2 & 0.14 & 0.68 &  \\
202 & MWISP G24.514$+$0.253 & 105.57 & 1.14 & 90  & 108 & 97  & 29  & 5.57 & 3.85 & 9.2  & 20.8 & 1.1 & 2.0 & 2.5 & 3.0  & 1.4 & 1.7 & 0.12 & 1.13 &  \\
203 & MWISP G24.342$+$0.299 & 109.53 & 0.72 & 90  & 104 & 96  & 131 & 6.86 & 3.41 & 13.0 & 20.8 & 1.4 & 2.2 & 2.2 & 0.9  & 1.4 & 1.1 & 0.15 & 0.71 &  \\
204 & MWISP G24.954$-$0.056 & 93.02  & 1.87 & 103 & 131 & 115 & 37  & 5.62 & 3.87 & 17.5 & 21.4 & 1.4 & 2.8 & 3.0 & 1.8  & 2.0 & 1.9 & 0.17 & 1.86 &  \\
205 & MWISP G24.312$-$0.059 & 89.37  & 2.70 & 98  & 195 & 124 & 109 & 5.24 & 4.01 & 11.3 & 21.3 & 1.6 & 2.8 & 3.4 & 4.3  & 1.8 & 2.1 & 0.14 & 2.70 &  \\
206 & MWISP G24.788$-$0.160 & 82.21  & 2.70 & 110 & 196 & 136 & 5   & 5.24 & 4.04 & 9.1  & 21.1 & 1.8 & 2.7 & 3.4 & 5.6  & 1.7 & 2.1 & 0.12 & 2.70 &  \\
207 & MWISP G24.354$+$0.005 & 113.50 & 1.72 & 141 & 229 & 170 & 64  & 7.19 & 3.37 & 11.7 & 21.1 & 3.0 & 3.1 & 3.3 & 1.5  & 1.6 & 1.2 & 0.14 & 1.71 &  \\
208 & MWISP G24.215$+$0.010 & 86.35  & 2.02 & 87  & 243 & 116 & 5   & 5.17 & 4.04 & 12.5 & 21.2 & 1.7 & 2.7 & 3.2 & 2.7  & 1.8 & 1.8 & 0.14 & 2.01 &  \\
209 & MWISP G24.418$-$0.096 & 108.10 & 2.44 & 91  & 133 & 106 & 130 & 6.09 & 3.62 & 12.1 & 21.3 & 1.5 & 2.7 & 3.3 & 3.6  & 1.9 & 2.1 & 0.14 & 2.44 &  \\
210 & MWISP G24.436$-$0.330 & 93.17  & 3.53 & 158 & 255 & 190 & 105 & 5.23 & 4.02 & 12.0 & 21.4 & 2.5 & 3.2 & 3.8 & 3.7  & 2.0 & 2.0 & 0.14 & 3.53 &  \\
211 & MWISP G24.485$+$0.490 & 102.38 & 1.08 & 68  & 130 & 85  & 144 & 5.64 & 3.82 & 12.3 & 20.9 & 1.1 & 2.1 & 2.4 & 1.9  & 1.6 & 1.7 & 0.14 & 1.07 &  \\
212 & MWISP G24.426$+$0.284 & 107.31 & 0.86 & 79  & 181 & 103 & 36  & 6.67 & 3.45 & 10.2 & 20.7 & 1.8 & 2.3 & 2.4 & 1.4  & 1.3 & 1.1 & 0.13 & 0.85 &  \\
213 & MWISP G24.441$+$0.348 & 117.92 & 2.41 & 159 & 364 & 206 & 116 & 6.78 & 3.43 & 8.9  & 21.1 & 3.9 & 3.3 & 3.7 & 2.5  & 1.6 & 1.3 & 0.12 & 2.41 &  \\
214 & MWISP G24.540$+$0.120 & 115.56 & 2.05 & 178 & 202 & 189 & 80  & 7.03 & 3.41 & 12.4 & 21.2 & 3.1 & 3.2 & 3.4 & 1.6  & 1.7 & 1.3 & 0.14 & 2.05 &  \\
215 & MWISP G24.298$-$0.197 & 80.49  & 1.82 & 80  & 139 & 98  & 29  & 5.01 & 4.13 & 10.1 & 21.0 & 1.1 & 2.3 & 2.9 & 4.4  & 1.6 & 2.1 & 0.13 & 1.82 &  \\
216 & MWISP G25.027$+$0.279 & 120.82 & 1.80 & 95  & 128 & 108 & 123 & 6.91 & 3.48 & 14.8 & 21.3 & 1.7 & 2.8 & 3.0 & 1.8  & 1.9 & 1.8 & 0.16 & 1.79 &  \\
217 & MWISP G24.335$-$0.168 & 113.02 & 2.43 & 128 & 380 & 172 & 67  & 6.94 & 3.39 & 11.3 & 21.2 & 3.6 & 3.4 & 3.7 & 1.9  & 1.8 & 1.4 & 0.14 & 2.43 &  \\
218 & MWISP G24.317$+$0.185 & 112.55 & 1.51 & 190 & 257 & 216 & 88  & 6.91 & 3.40 & 11.0 & 21.0 & 3.6 & 3.1 & 3.2 & 1.2  & 1.5 & 0.9 & 0.13 & 1.50 &  \\
219 & MWISP G24.481$+$0.002 & 106.66 & 1.19 & 117 & 250 & 150 & 127 & 5.70 & 3.79 & 15.1 & 21.1 & 2.3 & 2.8 & 2.8 & 1.0  & 1.6 & 1.1 & 0.16 & 1.18 &  \\
220 & MWISP G24.508$-$0.388 & 110.48 & 2.10 & 91  & 166 & 113 & 59  & 6.80 & 3.44 & 8.1  & 20.9 & 1.9 & 2.6 & 3.2 & 4.7  & 1.5 & 1.8 & 0.11 & 2.10 &  \\
221 & MWISP G24.505$-$0.245 & 101.75 & 2.10 & 76  & 76  & 76  & 76  & 5.76 & 3.76 & 13.1 & 21.3 & 0.8 & 2.3 & 2.9 & 3.7  & 2.0 & 2.5 & 0.15 & 2.09 &  \\
222 & MWISP G24.324$+$0.292 & 113.97 & 0.75 & 64  & 153 & 84  & 111 & 7.10 & 3.37 & 12.9 & 20.8 & 1.5 & 2.3 & 2.2 & 0.9  & 1.4 & 1.1 & 0.15 & 0.74 &  \\
223 & MWISP G24.342$+$0.215 & 110.64 & 0.93 & 67  & 138 & 85  & 119 & 6.70 & 3.44 & 10.6 & 20.8 & 1.3 & 2.2 & 2.4 & 1.7  & 1.4 & 1.4 & 0.13 & 0.92 &  \\
224 & MWISP G24.408$+$0.004 & 114.13 & 1.56 & 161 & 294 & 200 & 94  & 7.01 & 3.39 & 15.2 & 21.2 & 3.6 & 3.3 & 3.3 & 0.8  & 1.7 & 1.0 & 0.16 & 1.55 &  \\
225 & MWISP G24.669$+$0.089 & 110.46 & 1.56 & 93  & 132 & 108 & 153 & 6.52 & 3.52 & 10.4 & 21.0 & 1.6 & 2.5 & 2.9 & 2.7  & 1.6 & 1.7 & 0.13 & 1.55 &  \\
226 & MWISP G24.250$-$0.060 & 86.51  & 1.86 & 117 & 221 & 146 & 28  & 5.17 & 4.04 & 13.0 & 21.2 & 1.9 & 2.8 & 3.1 & 2.2  & 1.7 & 1.7 & 0.15 & 1.85 &  \\
227 & MWISP G24.529$+$0.056 & 117.78 & 2.09 & 82  & 117 & 95  & 1   & 7.25 & 3.39 & 14.6 & 21.3 & 1.5 & 2.8 & 3.1 & 2.2  & 1.9 & 2.0 & 0.15 & 2.08 &  \\
228 & MWISP G24.716$-$0.202 & 109.36 & 2.23 & 67  & 133 & 85  & 89  & 6.27 & 3.59 & 14.2 & 21.3 & 1.2 & 2.6 & 3.1 & 2.9  & 2.0 & 2.2 & 0.15 & 2.22 &  \\
229 & MWISP G24.556$-$0.209 & 95.72  & 2.72 & 114 & 214 & 142 & 154 & 5.54 & 3.87 & 13.7 & 21.4 & 2.0 & 3.0 & 3.5 & 2.8  & 1.9 & 2.0 & 0.15 & 2.72 &  \\
230 & MWISP G24.704$-$0.134 & 96.83  & 1.70 & 61  & 108 & 75  & 50  & 5.71 & 3.80 & 13.0 & 21.2 & 0.9 & 2.3 & 2.7 & 3.0  & 1.9 & 2.3 & 0.15 & 1.69 &  \\
231 & MWISP G24.294$+$0.002 & 88.26  & 1.72 & 135 & 255 & 168 & 126 & 5.22 & 4.01 & 10.0 & 21.0 & 2.3 & 2.7 & 3.1 & 2.5  & 1.5 & 1.5 & 0.13 & 1.72 &  \\
232 & MWISP G24.235$+$0.275 & 113.81 & 1.01 & 102 & 223 & 131 & 1   & 6.77 & 3.41 & 8.6  & 20.7 & 2.3 & 2.5 & 2.7 & 1.7  & 1.2 & 1.0 & 0.12 & 1.00 &  \\
233 & MWISP G24.270$-$0.329 & 90.48  & 2.22 & 187 & 241 & 209 & -13 & 5.09 & 4.09 & 5.6  & 20.7 & 2.5 & 2.5 & 3.4 & 7.8  & 1.2 & 1.6 & 0.10 & 2.22 &  \\
234 & MWISP G24.320$+$0.155 & 109.05 & 1.44 & 89  & 175 & 112 & 15  & 7.05 & 3.38 & 10.0 & 20.9 & 2.0 & 2.6 & 2.9 & 2.2  & 1.5 & 1.4 & 0.13 & 1.43 &  \\
235 & MWISP G24.688$+$0.446 & 112.38 & 2.11 & 192 & 411 & 246 & 116 & 6.21 & 3.61 & 21.1 & 21.5 & 4.2 & 3.8 & 3.6 & 0.7  & 2.0 & 1.1 & 0.19 & 2.10 &  \\
236 & MWISP G24.571$-$0.290 & 120.79 & 3.30 & 90  & 117 & 101 & 4   & 6.97 & 3.42 & 13.8 & 21.5 & 1.5 & 3.0 & 3.5 & 3.8  & 2.1 & 2.4 & 0.15 & 3.30 &  \\
237 & MWISP G24.391$+$0.218 & 110.00 & 2.17 & 88  & 140 & 105 & 106 & 7.66 & 3.37 & 10.3 & 21.1 & 1.9 & 2.8 & 3.3 & 3.2  & 1.7 & 1.8 & 0.13 & 2.17 &  \\
238 & MWISP G24.511$+$0.348 & 115.73 & 1.75 & 202 & 319 & 242 & 127 & 6.68 & 3.46 & 10.1 & 21.0 & 4.0 & 3.3 & 3.4 & 1.4  & 1.5 & 1.0 & 0.13 & 1.75 &  \\
239 & MWISP G24.165$+$0.020 & 98.58  & 2.09 & 82  & 141 & 100 & 126 & 5.59 & 3.81 & 13.9 & 21.3 & 1.3 & 2.6 & 3.1 & 2.9  & 1.9 & 2.1 & 0.15 & 2.08 &  \\
240 & MWISP G24.260$+$0.156 & 114.92 & 1.16 & 104 & 143 & 119 & 35  & 7.26 & 3.35 & 11.3 & 20.9 & 2.0 & 2.6 & 2.7 & 1.5  & 1.5 & 1.2 & 0.14 & 1.15 &  \\
241 & MWISP G25.058$+$0.078 & 106.20 & 1.06 & 112 & 149 & 126 & 129 & 6.05 & 3.70 & 13.5 & 21.0 & 1.7 & 2.5 & 2.6 & 1.2  & 1.5 & 1.3 & 0.15 & 1.05 &  \\
242 & MWISP G24.494$+$0.431 & 103.48 & 1.39 & 174 & 226 & 195 & 65  & 5.66 & 3.81 & 14.1 & 21.1 & 2.6 & 3.0 & 3.0 & 1.1  & 1.6 & 1.1 & 0.15 & 1.38 &  \\
243 & MWISP G24.391$+$0.483 & 102.39 & 0.67 & 70  & 167 & 91  & 42  & 5.62 & 3.82 & 9.0  & 20.5 & 1.3 & 1.9 & 2.1 & 1.7  & 1.1 & 1.1 & 0.12 & 0.66 &  \\
244 & MWISP G24.341$+$0.182 & 109.68 & 1.55 & 81  & 136 & 98  & 41  & 6.22 & 3.57 & 10.4 & 21.0 & 1.4 & 2.4 & 2.8 & 2.9  & 1.6 & 1.8 & 0.13 & 1.54 &  \\
245 & MWISP G24.461$+$0.018 & 117.15 & 7.51 & 75  & 128 & 91  & 93  & 7.21 & 3.38 & 10.7 & 21.7 & 1.5 & 3.2 & 4.2 & 12.1 & 2.3 & 3.1 & 0.13 & 7.51 &  \\
246 & MWISP G24.386$-$0.036 & 110.48 & 2.72 & 132 & 266 & 167 & 70  & 6.77 & 3.43 & 12.5 & 21.3 & 3.0 & 3.3 & 3.7 & 2.2  & 1.9 & 1.6 & 0.14 & 2.72 &  \\
247 & MWISP G24.485$+$0.115 & 112.54 & 1.98 & 110 & 110 & 110 & 90  & 6.82 & 3.43 & 15.1 & 21.3 & 1.6 & 2.8 & 3.1 & 2.0  & 1.9 & 1.9 & 0.16 & 1.97 &  \\
248 & MWISP G24.472$-$0.208 & 96.51  & 1.72 & 76  & 142 & 95  & 61  & 5.55 & 3.86 & 14.4 & 21.2 & 1.2 & 2.5 & 2.9 & 2.3  & 1.8 & 2.0 & 0.15 & 1.71 &  \\
249 & MWISP G24.326$+$0.357 & 114.91 & 0.68 & 91  & 200 & 117 & 77  & 6.69 & 3.44 & 11.6 & 20.7 & 2.0 & 2.4 & 2.3 & 0.8  & 1.3 & 0.7 & 0.14 & 0.67 &  \\
250 & MWISP G24.180$+$0.265 & 110.95 & 1.19 & 100 & 233 & 130 & 48  & 7.10 & 3.36 & 9.9  & 20.8 & 2.5 & 2.7 & 2.9 & 1.5  & 1.4 & 1.1 & 0.13 & 1.18 &  \\
251 & MWISP G24.402$+$0.023 & 87.63  & 1.46 & 136 & 136 & 136 & 65  & 5.25 & 4.01 & 18.1 & 21.3 & 1.6 & 2.8 & 2.9 & 1.3  & 1.8 & 1.6 & 0.17 & 1.45 &  \\
252 & MWISP G24.374$-$0.002 & 118.58 & 1.83 & 196 & 264 & 223 & 41  & 7.31 & 3.37 & 14.8 & 21.3 & 3.9 & 3.5 & 3.4 & 0.9  & 1.8 & 1.0 & 0.16 & 1.82 &  \\
253 & MWISP G24.823$+$0.123 & 105.39 & 1.98 & 85  & 132 & 101 & 73  & 6.00 & 3.70 & 16.1 & 21.3 & 1.4 & 2.7 & 3.0 & 2.1  & 2.0 & 2.0 & 0.16 & 1.97 &  \\
254 & MWISP G24.752$-$0.190 & 92.22  & 2.88 & 117 & 254 & 150 & 40  & 5.43 & 3.94 & 9.2  & 21.2 & 2.2 & 2.9 & 3.6 & 4.9  & 1.7 & 1.9 & 0.12 & 2.88 &  \\
255 & MWISP G24.376$+$0.434 & 102.54 & 0.84 & 73  & 126 & 89  & 113 & 5.60 & 3.83 & 7.3  & 20.5 & 1.1 & 1.7 & 2.2 & 3.2  & 1.1 & 1.5 & 0.11 & 0.83 &  \\
256 & MWISP G24.766$+$0.116 & 101.44 & 1.90 & 106 & 174 & 128 & 75  & 5.88 & 3.74 & 19.4 & 21.4 & 1.8 & 3.0 & 3.1 & 1.4  & 2.0 & 1.7 & 0.18 & 1.89 &  \\
257 & MWISP G24.450$+$0.139 & 119.68 & 1.94 & 90  & 130 & 105 & 78  & 7.27 & 3.38 & 18.3 & 21.4 & 1.7 & 3.0 & 3.1 & 1.4  & 2.0 & 1.8 & 0.17 & 1.93 & 
\enddata
% \tablecomments{第(1)列：序号。第(2)列：由MWISP项目定义的源名。第(3)-(4)列：中心速度和线宽。第(5)-(8)：团块的长轴、短轴、直径和方向。第(9)-(10)列：日心距和银心距。第(11)列：激发温度。第(12)列：氢气柱密度。第(13)列：有效半径。第(14)列：团块质量。第(15)列：维里质量。第(16)列：维里参数。第(17)列：表面密度。第(18)列：氢分子的数密度。第(19)-(20)列：热线宽和非热线宽。第(21)列：团块是否具备形成大质量恒星的潜力（见第4.5节）。}
\tablecomments{Column (1): clump number. Column (2): source name defined by the Galactic Coordinates. Columns (3) and (4): central velocity and linewidth of each clump. Columns (5) -- (8): major axis, minor axis, diameter and positional angle of the clumps. Columns (9) and (10): heliocentric distance and Galactocentric distance. Column (11): excitation temperature. Column (12): hydrogen column density. Column (13): effective radius. Column (14): mass of clumps. Column (15): virial mass. Column (16): virial parameter. Column (17): surface density. Column (18): number density of hydrogen molecules. Columns (19) and (20): thermal and non-thermal linewidth. Columns (21): whether the clumps have the potential to form massive stars (see subsection \ref{subsec:4.1.5}).}
\label{appendix:the parameters of 12CO clumps}
\end{deluxetable*}
\end{longrotatetable}

==> the_parameters_of_13CO_clumps.tex <==
\begin{longrotatetable}
\addtolength{\tabcolsep}{-1.5pt}
\begin{deluxetable*}{ccccccccccccccccccccc}
\tablecaption{The parameters of $^{13}$CO clumps}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{Number} & \colhead{Source} & \colhead{$V_{\text{lsr}}$} & \colhead{$\Delta v$} & \colhead{$\theta_{\text{a}}$} & \colhead{$\theta_{\text{b}}$} & \colhead{$\theta_{\text{fwhm}}$} & \colhead{P.A.} & \colhead{Distance} & \colhead{$R_{\text{GC}}$} & \colhead{$T_{\text{ex}}$} & \colhead{log($N_{\text{H$_2$}}$)} & \colhead{$R_{\text{eff}}$} & \colhead{log($M_{\text{clump}}$)} & \colhead{log($M_{\text{vir}}$)} & \colhead{$\alpha_{\text{vir}}$} & \colhead{log($\Sigma$)} & \colhead{log($n_{\text{H$_2$}}$)} & \colhead{$\Delta v_{\text{th}}$} & \colhead{$\Delta v_{\text{nth}}$} & \colhead{Potential} \\
\colhead{} & \colhead{} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{($\arcsec$)} & \colhead{($\arcsec$)} & \colhead{($\arcsec$)} & \colhead{($\arcdeg$)} & \colhead{(kpc)} & \colhead{(kpc)} & \colhead{(K)} & \colhead{(cm$^{-2}$)} & \colhead{(pc)} & \colhead{($M_{\sun}$)} & \colhead{($M_{\sun}$)} & \colhead{} & \colhead{($M_{\sun}$ pc$^{-2}$)} & \colhead{(cm$^{-3}$)} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{}
\decimalcolnumbers
}
\startdata
1   & MWISP G24.473$+$0.480 & 102.38 & 2.84 & 108 & 191 & 133 & 83  & 5.64 & 3.82 & 13.8 & 21.7 & 1.8 & 3.3 & 3.5 & 1.6  & 2.3 & 3.6 & 0.15 & 2.84 &            \\
2   & MWISP G24.670$-$0.156 & 112.34 & 2.54 & 84  & 213 & 111 & 112 & 6.69 & 3.48 & 14.0 & 21.6 & 2.0 & 3.3 & 3.4 & 1.4  & 2.2 & 3.4 & 0.15 & 2.54 &            \\
3   & MWISP G24.780$+$0.088 & 110.13 & 2.28 & 154 & 215 & 177 & 129 & 6.40 & 3.56 & 18.7 & 21.8 & 2.7 & 3.7 & 3.5 & 0.5  & 2.4 & 3.5 & 0.17 & 2.27 &            \\
4   & MWISP G24.454$+$0.191 & 118.82 & 2.02 & 100 & 145 & 116 & 39  & 7.23 & 3.38 & 10.6 & 21.2 & 1.9 & 2.8 & 3.2 & 2.4  & 1.8 & 3.0 & 0.13 & 2.02 &            \\
5   & MWISP G24.490$-$0.042 & 110.49 & 2.56 & 99  & 116 & 107 & 86  & 6.68 & 3.46 & 10.2 & 21.1 & 1.5 & 2.6 & 3.3 & 5.5  & 1.7 & 3.1 & 0.13 & 2.56 &            \\
6   & MWISP G24.559$-$0.217 & 99.67  & 1.50 & 131 & 131 & 131 & 63  & 5.73 & 3.78 & 15.5 & 21.3 & 1.7 & 2.9 & 2.9 & 1.1  & 1.9 & 3.2 & 0.16 & 1.49 &            \\
7   & MWISP G24.552$-$0.246 & 98.22  & 1.88 & 80  & 117 & 94  & 39  & 5.65 & 3.82 & 12.9 & 21.3 & 1.1 & 2.5 & 2.9 & 2.5  & 1.9 & 3.4 & 0.14 & 1.87 &            \\
8   & MWISP G24.232$+$0.227 & 113.83 & 2.10 & 159 & 292 & 197 & 46  & 7.21 & 3.35 & 10.2 & 21.2 & 3.7 & 3.4 & 3.5 & 1.4  & 1.8 & 2.7 & 0.13 & 2.10 &            \\
9   & MWISP G24.445$+$0.506 & 100.88 & 1.83 & 91  & 98  & 94  & -26 & 5.60 & 3.83 & 13.9 & 21.3 & 1.1 & 2.5 & 2.9 & 2.5  & 1.9 & 3.4 & 0.15 & 1.82 &            \\
10  & MWISP G24.436$+$0.260 & 117.01 & 1.75 & 106 & 193 & 132 & 97  & 7.16 & 3.38 & 9.9  & 21.0 & 2.3 & 2.8 & 3.2 & 2.3  & 1.6 & 2.8 & 0.13 & 1.75 &            \\
11  & MWISP G24.470$+$0.488 & 104.03 & 1.75 & 99  & 134 & 113 & 83  & 5.68 & 3.80 & 13.6 & 21.4 & 1.4 & 2.8 & 3.0 & 1.3  & 2.0 & 3.4 & 0.15 & 1.74 &            \\
12  & MWISP G24.506$-$0.231 & 99.55  & 2.61 & 86  & 143 & 104 & 106 & 5.70 & 3.79 & 15.4 & 21.5 & 1.4 & 2.8 & 3.3 & 2.9  & 2.1 & 3.5 & 0.16 & 2.61 &            \\
13  & MWISP G24.722$+$0.082 & 109.68 & 1.68 & 70  & 108 & 83  & 134 & 6.40 & 3.55 & 12.5 & 21.3 & 1.1 & 2.5 & 2.8 & 1.9  & 1.9 & 3.4 & 0.14 & 1.67 &            \\
14  & MWISP G24.421$+$0.117 & 112.67 & 2.44 & 130 & 244 & 162 & 85  & 6.87 & 3.41 & 14.9 & 21.8 & 2.8 & 3.7 & 3.5 & 0.7  & 2.3 & 3.4 & 0.15 & 2.44 &            \\
15  & MWISP G24.539$-$0.135 & 94.59  & 1.92 & 102 & 222 & 131 & 27  & 5.51 & 3.88 & 10.9 & 21.2 & 1.9 & 2.9 & 3.2 & 2.0  & 1.8 & 3.1 & 0.13 & 1.92 &            \\
16  & MWISP G24.502$+$0.453 & 103.67 & 1.58 & 95  & 153 & 114 & 2   & 5.67 & 3.80 & 12.8 & 21.4 & 1.5 & 2.8 & 2.9 & 1.2  & 2.0 & 3.3 & 0.14 & 1.57 &            \\
17  & MWISP G24.542$-$0.282 & 96.72  & 1.96 & 88  & 255 & 117 & -16 & 5.54 & 3.87 & 12.1 & 21.3 & 1.9 & 2.9 & 3.2 & 1.9  & 1.9 & 3.1 & 0.14 & 1.96 &            \\
18  & MWISP G24.635$-$0.110 & 112.20 & 2.14 & 113 & 146 & 126 & -5  & 6.73 & 3.46 & 9.9  & 21.1 & 1.9 & 2.7 & 3.3 & 3.6  & 1.6 & 2.9 & 0.13 & 2.14 &            \\
19  & MWISP G24.796$+$0.097 & 106.70 & 2.92 & 102 & 175 & 124 & 122 & 6.06 & 3.67 & 15.9 & 21.8 & 1.8 & 3.4 & 3.5 & 1.3  & 2.4 & 3.7 & 0.16 & 2.92 & \checkmark \\
20  & MWISP G24.532$-$0.210 & 101.37 & 1.97 & 66  & 139 & 84  & 3   & 5.79 & 3.75 & 18.1 & 21.7 & 1.1 & 3.0 & 3.0 & 0.9  & 2.4 & 3.9 & 0.17 & 1.96 &            \\
21  & MWISP G24.435$+$0.172 & 116.49 & 2.32 & 156 & 292 & 195 & 82  & 7.22 & 3.38 & 13.4 & 21.5 & 3.6 & 3.7 & 3.6 & 0.9  & 2.1 & 3.0 & 0.15 & 2.32 &            \\
22  & MWISP G24.843$-$0.027 & 104.52 & 1.98 & 114 & 153 & 130 & 0   & 5.99 & 3.70 & 13.4 & 21.2 & 1.8 & 2.8 & 3.2 & 2.2  & 1.8 & 3.1 & 0.15 & 1.97 &            \\
23  & MWISP G24.366$+$0.043 & 117.32 & 2.64 & 183 & 308 & 222 & 104 & 7.30 & 3.36 & 15.8 & 21.6 & 4.1 & 3.9 & 3.8 & 0.8  & 2.2 & 3.1 & 0.16 & 2.64 &            \\
24  & MWISP G24.177$+$0.401 & 94.72  & 1.34 & 103 & 103 & 103 & 116 & 5.27 & 3.98 & 8.3  & 20.9 & 1.1 & 2.1 & 2.6 & 3.4  & 1.5 & 3.0 & 0.11 & 1.34 &            \\
25  & MWISP G24.739$+$0.150 & 107.20 & 2.39 & 90  & 156 & 110 & 130 & 6.05 & 3.67 & 17.0 & 21.8 & 1.6 & 3.3 & 3.3 & 0.9  & 2.4 & 3.8 & 0.16 & 2.38 & \checkmark \\
26  & MWISP G24.204$-$0.259 & 93.40  & 1.84 & 102 & 109 & 105 & 142 & 5.24 & 4.00 & 6.3  & 20.6 & 1.2 & 1.8 & 2.9 & 12.6 & 1.2 & 2.7 & 0.10 & 1.84 &            \\
27  & MWISP G24.414$+$0.116 & 110.36 & 2.28 & 122 & 206 & 148 & 74  & 7.22 & 3.37 & 14.4 & 21.7 & 2.6 & 3.6 & 3.5 & 0.7  & 2.3 & 3.4 & 0.15 & 2.28 &            \\
28  & MWISP G24.438$-$0.272 & 95.30  & 1.35 & 83  & 196 & 109 & 17  & 5.41 & 3.93 & 12.9 & 21.1 & 1.5 & 2.5 & 2.8 & 1.7  & 1.7 & 3.0 & 0.14 & 1.34 &            \\
29  & MWISP G24.334$+$0.146 & 111.68 & 2.69 & 102 & 227 & 132 & -9  & 6.84 & 3.41 & 10.3 & 21.1 & 2.4 & 3.0 & 3.6 & 4.0  & 1.7 & 2.9 & 0.13 & 2.69 &            \\
30  & MWISP G24.131$+$0.253 & 113.15 & 1.57 & 95  & 215 & 123 & -4  & 7.33 & 3.33 & 11.2 & 21.1 & 2.4 & 2.9 & 3.1 & 1.4  & 1.7 & 2.9 & 0.13 & 1.56 &            \\
31  & MWISP G24.144$-$0.109 & 79.92  & 1.59 & 107 & 154 & 124 & 57  & 5.08 & 4.08 & 9.9  & 20.9 & 1.4 & 2.3 & 2.9 & 3.9  & 1.5 & 2.9 & 0.13 & 1.59 &            \\
32  & MWISP G24.864$+$0.007 & 108.53 & 1.93 & 95  & 189 & 120 & 91  & 6.15 & 3.65 & 14.6 & 21.6 & 1.8 & 3.2 & 3.2 & 0.9  & 2.2 & 3.4 & 0.15 & 1.92 &            \\
33  & MWISP G24.953$-$0.053 & 92.58  & 1.37 & 78  & 112 & 91  & 27  & 5.59 & 3.88 & 15.8 & 21.5 & 1.1 & 2.7 & 2.6 & 0.9  & 2.1 & 3.7 & 0.16 & 1.36 &            \\
34  & MWISP G24.759$+$0.089 & 108.18 & 1.51 & 106 & 174 & 128 & 86  & 5.44 & 3.94 & 17.7 & 21.7 & 1.7 & 3.2 & 2.9 & 0.5  & 2.2 & 3.6 & 0.17 & 1.50 &            \\
35  & MWISP G24.122$+$0.125 & 112.37 & 1.49 & 92  & 157 & 112 & 13  & 7.41 & 3.33 & 11.5 & 21.1 & 2.0 & 2.8 & 3.0 & 1.6  & 1.7 & 2.9 & 0.13 & 1.48 &            \\
36  & MWISP G24.479$+$0.481 & 100.55 & 1.58 & 70  & 158 & 91  & 87  & 5.59 & 3.84 & 12.5 & 21.3 & 1.2 & 2.6 & 2.8 & 1.5  & 1.9 & 3.4 & 0.14 & 1.57 &            \\
37  & MWISP G24.451$+$0.211 & 121.28 & 2.61 & 172 & 227 & 194 & 101 & 7.19 & 3.38 & 9.4  & 21.3 & 3.3 & 3.4 & 3.7 & 1.9  & 1.9 & 2.9 & 0.12 & 2.61 &            \\
38  & MWISP G24.531$+$0.320 & 112.31 & 1.91 & 126 & 222 & 154 & 108 & 6.71 & 3.46 & 8.8  & 20.8 & 2.6 & 2.7 & 3.3 & 3.9  & 1.4 & 2.5 & 0.12 & 1.91 &            \\
39  & MWISP G24.790$+$0.098 & 112.49 & 2.14 & 89  & 102 & 95  & 114 & 6.64 & 3.50 & 17.0 & 21.7 & 1.3 & 3.1 & 3.1 & 1.1  & 2.3 & 3.8 & 0.16 & 2.13 &            \\
40  & MWISP G24.839$+$0.034 & 105.20 & 1.89 & 117 & 231 & 148 & 35  & 6.02 & 3.69 & 16.0 & 21.7 & 2.3 & 3.5 & 3.2 & 0.5  & 2.3 & 3.5 & 0.16 & 1.88 &            \\
41  & MWISP G24.564$+$0.339 & 108.87 & 2.36 & 164 & 310 & 205 & 159 & 6.55 & 3.50 & 13.8 & 21.5 & 3.5 & 3.6 & 3.6 & 1.0  & 2.0 & 3.0 & 0.15 & 2.36 &            \\
42  & MWISP G24.146$+$0.397 & 93.43  & 2.25 & 88  & 161 & 109 & 8   & 5.21 & 4.01 & 7.3  & 20.8 & 1.4 & 2.1 & 3.2 & 10.4 & 1.4 & 2.8 & 0.11 & 2.25 &            \\
43  & MWISP G24.334$+$0.061 & 114.17 & 2.27 & 153 & 221 & 178 & 27  & 7.22 & 3.36 & 19.8 & 21.8 & 3.1 & 3.8 & 3.5 & 0.6  & 2.3 & 3.3 & 0.18 & 2.26 &            \\
44  & MWISP G24.540$-$0.251 & 96.90  & 1.74 & 59  & 78  & 66  & 61  & 5.57 & 3.85 & 14.4 & 21.3 & 0.6 & 2.3 & 2.6 & 2.1  & 2.2 & 4.0 & 0.15 & 1.73 &            \\
45  & MWISP G24.415$+$0.105 & 114.99 & 2.06 & 197 & 529 & 261 & 115 & 7.22 & 3.37 & 15.3 & 21.8 & 5.6 & 4.3 & 3.7 & 0.3  & 2.3 & 3.1 & 0.16 & 2.05 &            \\
46  & MWISP G24.360$+$0.274 & 112.01 & 1.54 & 126 & 171 & 144 & 123 & 7.05 & 3.38 & 10.5 & 21.0 & 2.4 & 2.8 & 3.1 & 2.0  & 1.5 & 2.7 & 0.13 & 1.53 &            \\
47  & MWISP G24.433$+$0.478 & 101.72 & 1.23 & 132 & 136 & 134 & 111 & 5.61 & 3.83 & 19.2 & 21.5 & 1.7 & 3.1 & 2.7 & 0.5  & 2.1 & 3.4 & 0.17 & 1.22 &            \\
48  & MWISP G24.259$+$0.166 & 112.51 & 2.10 & 84  & 135 & 101 & 155 & 7.18 & 3.36 & 11.1 & 21.4 & 1.6 & 2.9 & 3.2 & 1.8  & 2.0 & 3.3 & 0.13 & 2.10 &            \\
49  & MWISP G24.802$+$0.032 & 107.19 & 1.85 & 76  & 193 & 100 & -15 & 6.09 & 3.66 & 17.0 & 21.7 & 1.6 & 3.2 & 3.1 & 0.8  & 2.2 & 3.6 & 0.16 & 1.84 &            \\
50  & MWISP G24.655$-$0.105 & 114.50 & 2.44 & 91  & 113 & 100 & 61  & 6.91 & 3.44 & 9.7  & 21.1 & 1.5 & 2.5 & 3.3 & 5.5  & 1.7 & 3.1 & 0.12 & 2.44 &            \\
51  & MWISP G24.799$-$0.096 & 80.31  & 1.52 & 122 & 169 & 140 & 77  & 5.26 & 4.03 & 9.9  & 21.0 & 1.7 & 2.5 & 2.9 & 2.6  & 1.5 & 2.9 & 0.13 & 1.51 &            \\
52  & MWISP G24.777$-$0.027 & 108.84 & 1.99 & 104 & 247 & 136 & 36  & 5.32 & 4.00 & 15.4 & 21.6 & 2.0 & 3.2 & 3.2 & 1.0  & 2.1 & 3.4 & 0.16 & 1.98 &            \\
53  & MWISP G24.649$+$0.384 & 109.67 & 1.88 & 185 & 284 & 220 & 139 & 5.79 & 3.76 & 13.7 & 21.4 & 3.1 & 3.4 & 3.4 & 0.9  & 1.9 & 3.0 & 0.15 & 1.87 &            \\
54  & MWISP G24.469$+$0.296 & 121.28 & 2.08 & 94  & 153 & 113 & 124 & 6.93 & 3.41 & 9.6  & 21.0 & 1.8 & 2.6 & 3.2 & 4.4  & 1.6 & 2.8 & 0.12 & 2.08 &            \\
55  & MWISP G24.427$+$0.328 & 114.50 & 2.13 & 101 & 296 & 135 & 96  & 6.68 & 3.45 & 9.1  & 20.9 & 2.7 & 2.8 & 3.4 & 3.8  & 1.5 & 2.6 & 0.12 & 2.13 &            \\
56  & MWISP G24.197$+$0.407 & 95.59  & 1.96 & 102 & 116 & 108 & 88  & 5.31 & 3.96 & 9.1  & 21.1 & 1.2 & 2.4 & 3.0 & 3.7  & 1.8 & 3.2 & 0.12 & 1.96 &            \\
57  & MWISP G24.453$-$0.285 & 96.55  & 1.19 & 94  & 142 & 111 & 155 & 5.48 & 3.89 & 15.4 & 21.3 & 1.4 & 2.7 & 2.6 & 0.8  & 1.9 & 3.3 & 0.16 & 1.18 &            \\
58  & MWISP G24.481$+$0.117 & 112.18 & 2.47 & 93  & 108 & 100 & 43  & 6.79 & 3.44 & 14.6 & 21.5 & 1.4 & 2.9 & 3.3 & 2.0  & 2.1 & 3.5 & 0.15 & 2.47 &            \\
59  & MWISP G24.386$+$0.198 & 112.35 & 2.30 & 206 & 416 & 261 & 85  & 6.79 & 3.42 & 10.3 & 21.1 & 4.7 & 3.5 & 3.7 & 1.6  & 1.7 & 2.5 & 0.13 & 2.30 &            \\
60  & MWISP G24.541$+$0.487 & 102.07 & 1.69 & 132 & 268 & 167 & 127 & 5.65 & 3.82 & 11.0 & 20.9 & 2.5 & 2.8 & 3.2 & 2.6  & 1.5 & 2.6 & 0.13 & 1.68 &            \\
61  & MWISP G24.729$+$0.153 & 108.86 & 1.73 & 76  & 76  & 76  & -39 & 6.24 & 3.60 & 16.3 & 21.6 & 0.9 & 2.7 & 2.7 & 1.1  & 2.3 & 4.0 & 0.16 & 1.72 &            \\
62  & MWISP G24.482$+$0.157 & 118.15 & 1.57 & 65  & 101 & 77  & 144 & 7.23 & 3.38 & 12.5 & 21.1 & 1.1 & 2.4 & 2.8 & 2.4  & 1.8 & 3.3 & 0.14 & 1.56 &            \\
63  & MWISP G24.364$+$0.084 & 97.06  & 1.64 & 98  & 126 & 109 & 150 & 5.61 & 3.82 & 11.4 & 21.0 & 1.3 & 2.4 & 2.9 & 3.0  & 1.6 & 3.1 & 0.13 & 1.63 &            \\
64  & MWISP G24.541$+$0.500 & 109.34 & 1.67 & 86  & 99  & 92  & 85  & 6.03 & 3.66 & 8.5  & 20.7 & 1.1 & 2.0 & 2.8 & 6.4  & 1.4 & 2.9 & 0.12 & 1.67 &            \\
65  & MWISP G24.674$-$0.156 & 114.33 & 2.08 & 79  & 158 & 100 & 138 & 6.86 & 3.45 & 14.0 & 21.5 & 1.7 & 3.1 & 3.2 & 1.3  & 2.1 & 3.5 & 0.15 & 2.07 &            \\
66  & MWISP G24.241$+$0.006 & 90.73  & 1.47 & 74  & 107 & 86  & -36 & 5.27 & 3.98 & 12.2 & 21.3 & 0.9 & 2.4 & 2.6 & 1.5  & 2.0 & 3.6 & 0.14 & 1.46 &            \\
67  & MWISP G24.506$-$0.102 & 94.74  & 2.32 & 101 & 137 & 115 & 53  & 5.52 & 3.88 & 12.2 & 21.3 & 1.4 & 2.7 & 3.2 & 3.2  & 1.9 & 3.3 & 0.14 & 2.32 &            \\
68  & MWISP G24.134$-$0.110 & 69.99  & 1.37 & 60  & 119 & 75  & 88  & 5.11 & 4.06 & 9.7  & 21.0 & 0.8 & 2.0 & 2.5 & 3.0  & 1.7 & 3.3 & 0.12 & 1.36 &            \\
69  & MWISP G24.763$+$0.133 & 109.64 & 1.46 & 104 & 185 & 128 & 122 & 6.32 & 3.58 & 20.0 & 21.7 & 2.0 & 3.4 & 2.9 & 0.4  & 2.3 & 3.5 & 0.18 & 1.45 &            \\
70  & MWISP G24.243$+$0.202 & 112.50 & 1.23 & 92  & 92  & 92  & -11 & 7.22 & 3.35 & 10.6 & 21.2 & 1.3 & 2.6 & 2.6 & 0.9  & 1.9 & 3.3 & 0.13 & 1.22 &            \\
71  & MWISP G24.950$+$0.467 & 111.33 & 1.49 & 79  & 106 & 90  & 1   & 6.16 & 3.65 & 14.4 & 21.2 & 1.1 & 2.5 & 2.7 & 1.8  & 1.9 & 3.4 & 0.15 & 1.48 &            \\
72  & MWISP G24.494$+$0.319 & 117.15 & 2.57 & 94  & 205 & 121 & 124 & 6.80 & 3.43 & 9.3  & 21.0 & 2.1 & 2.7 & 3.5 & 5.4  & 1.6 & 2.8 & 0.12 & 2.57 &            \\
73  & MWISP G24.362$+$0.297 & 113.99 & 1.44 & 108 & 215 & 137 & 113 & 7.08 & 3.38 & 11.7 & 21.1 & 2.5 & 3.0 & 3.0 & 1.2  & 1.7 & 2.8 & 0.14 & 1.43 &            \\
74  & MWISP G24.697$+$0.015 & 108.99 & 1.84 & 173 & 216 & 191 & 79  & 5.58 & 3.86 & 13.6 & 21.3 & 2.5 & 3.2 & 3.3 & 1.3  & 1.9 & 3.0 & 0.15 & 1.83 &            \\
75  & MWISP G24.470$-$0.047 & 108.84 & 1.84 & 92  & 212 & 119 & -2  & 6.17 & 3.60 & 9.0  & 20.9 & 1.9 & 2.5 & 3.1 & 4.2  & 1.4 & 2.7 & 0.12 & 1.84 &            \\
76  & MWISP G24.857$+$0.070 & 109.01 & 1.89 & 66  & 130 & 83  & 85  & 5.29 & 4.02 & 13.6 & 21.6 & 1.0 & 2.8 & 2.9 & 1.2  & 2.3 & 3.8 & 0.15 & 1.88 &            \\
77  & MWISP G24.267$+$0.097 & 99.55  & 1.72 & 142 & 167 & 153 & -19 & 5.69 & 3.77 & 11.7 & 21.2 & 2.0 & 2.9 & 3.1 & 1.7  & 1.8 & 3.0 & 0.14 & 1.71 &            \\
78  & MWISP G24.761$+$0.493 & 105.36 & 1.94 & 113 & 145 & 126 & 52  & 5.73 & 3.80 & 20.5 & 21.9 & 1.6 & 3.4 & 3.1 & 0.5  & 2.4 & 3.8 & 0.18 & 1.93 & \checkmark \\
79  & MWISP G24.295$-$0.195 & 80.46  & 1.38 & 72  & 111 & 86  & 22  & 5.07 & 4.10 & 10.1 & 20.7 & 0.9 & 1.8 & 2.6 & 5.3  & 1.4 & 3.0 & 0.13 & 1.37 &            \\
80  & MWISP G24.180$+$0.050 & 109.51 & 2.80 & 134 & 321 & 175 & 5   & 7.49 & 3.34 & 14.0 & 21.5 & 3.7 & 3.7 & 3.8 & 1.3  & 2.0 & 3.0 & 0.15 & 2.80 &            \\
81  & MWISP G24.116$+$0.014 & 100.88 & 1.90 & 87  & 87  & 87  & 84  & 5.58 & 3.81 & 14.6 & 21.5 & 1.0 & 2.7 & 2.9 & 1.5  & 2.2 & 3.8 & 0.15 & 1.89 &            \\
82  & MWISP G24.162$-$0.007 & 86.43  & 1.27 & 62  & 146 & 81  & -6  & 5.16 & 4.04 & 13.6 & 21.4 & 1.0 & 2.5 & 2.5 & 1.0  & 2.0 & 3.6 & 0.15 & 1.26 &            \\
83  & MWISP G24.660$-$0.303 & 115.14 & 1.64 & 96  & 139 & 112 & 122 & 6.73 & 3.47 & 13.2 & 21.3 & 1.7 & 2.9 & 3.0 & 1.3  & 1.9 & 3.2 & 0.14 & 1.63 &            \\
84  & MWISP G24.313$+$0.161 & 113.01 & 1.19 & 122 & 137 & 129 & 170 & 7.18 & 3.36 & 9.7  & 20.9 & 2.1 & 2.6 & 2.8 & 1.6  & 1.5 & 2.7 & 0.12 & 1.18 &            \\
85  & MWISP G24.598$+$0.441 & 107.85 & 1.49 & 63  & 166 & 83  & 79  & 5.92 & 3.71 & 14.5 & 21.4 & 1.3 & 2.8 & 2.8 & 1.0  & 2.1 & 3.5 & 0.15 & 1.48 &            \\
86  & MWISP G24.208$-$0.323 & 88.77  & 1.89 & 133 & 180 & 151 & 100 & 5.04 & 4.11 & 5.0  & 20.5 & 1.8 & 2.1 & 3.1 & 10.8 & 1.1 & 2.4 & 0.09 & 1.89 &            \\
87  & MWISP G24.444$+$0.438 & 102.53 & 1.49 & 149 & 272 & 185 & 17  & 5.63 & 3.82 & 6.8  & 20.6 & 2.7 & 2.5 & 3.1 & 3.9  & 1.2 & 2.3 & 0.10 & 1.49 &            \\
88  & MWISP G24.747$+$0.176 & 108.19 & 1.78 & 60  & 120 & 76  & 51  & 5.45 & 3.93 & 18.4 & 21.8 & 0.9 & 3.0 & 2.8 & 0.7  & 2.5 & 4.1 & 0.17 & 1.77 & \checkmark \\
89  & MWISP G24.295$+$0.209 & 112.51 & 1.64 & 105 & 163 & 125 & 153 & 7.15 & 3.36 & 12.0 & 21.4 & 2.1 & 3.1 & 3.1 & 0.9  & 2.0 & 3.2 & 0.14 & 1.63 &            \\
90  & MWISP G24.686$+$0.440 & 111.38 & 1.71 & 128 & 208 & 154 & 128 & 5.88 & 3.73 & 18.6 & 21.7 & 2.2 & 3.4 & 3.1 & 0.5  & 2.3 & 3.5 & 0.17 & 1.70 &            \\
91  & MWISP G24.303$+$0.264 & 113.00 & 1.64 & 133 & 281 & 170 & 168 & 7.11 & 3.37 & 12.8 & 21.2 & 3.2 & 3.2 & 3.3 & 1.0  & 1.7 & 2.8 & 0.14 & 1.63 &            \\
92  & MWISP G24.494$+$0.300 & 110.68 & 1.40 & 161 & 212 & 181 & 33  & 6.01 & 3.66 & 9.3  & 20.8 & 2.6 & 2.7 & 3.0 & 2.3  & 1.3 & 2.5 & 0.12 & 1.39 &            \\
93  & MWISP G24.394$+$0.172 & 110.51 & 1.97 & 181 & 230 & 201 & 155 & 6.09 & 3.62 & 12.1 & 21.1 & 2.9 & 3.1 & 3.4 & 2.0  & 1.7 & 2.7 & 0.14 & 1.97 &            \\
94  & MWISP G24.360$+$0.210 & 114.49 & 1.50 & 136 & 178 & 153 & 162 & 7.15 & 3.37 & 9.7  & 20.9 & 2.5 & 2.8 & 3.1 & 2.1  & 1.5 & 2.6 & 0.12 & 1.49 &            \\
95  & MWISP G24.789$+$0.078 & 108.68 & 1.65 & 58  & 149 & 76  & 122 & 5.44 & 3.94 & 17.7 & 21.6 & 1.0 & 2.8 & 2.8 & 0.9  & 2.3 & 3.8 & 0.17 & 1.64 &            \\
96  & MWISP G24.273$+$0.444 & 96.56  & 1.95 & 112 & 131 & 120 & 39  & 5.38 & 3.93 & 8.2  & 20.8 & 1.4 & 2.2 & 3.1 & 7.4  & 1.4 & 2.8 & 0.11 & 1.95 &            \\
97  & MWISP G24.412$+$0.065 & 113.34 & 1.92 & 73  & 145 & 93  & 76  & 6.96 & 3.40 & 21.8 & 21.9 & 1.5 & 3.4 & 3.1 & 0.5  & 2.5 & 3.9 & 0.19 & 1.91 & \checkmark \\
98  & MWISP G24.524$+$0.121 & 115.99 & 1.34 & 116 & 163 & 134 & 154 & 7.19 & 3.39 & 9.0  & 20.7 & 2.2 & 2.5 & 2.9 & 2.6  & 1.3 & 2.5 & 0.12 & 1.33 &            \\
99  & MWISP G24.368$+$0.258 & 110.20 & 1.12 & 158 & 213 & 180 & 111 & 5.90 & 3.69 & 12.0 & 20.9 & 2.5 & 2.7 & 2.8 & 1.2  & 1.4 & 2.6 & 0.14 & 1.11 &            \\
100 & MWISP G24.626$+$0.181 & 114.82 & 2.23 & 99  & 123 & 109 & 35  & 6.86 & 3.44 & 10.9 & 21.2 & 1.6 & 2.7 & 3.2 & 3.2  & 1.8 & 3.1 & 0.13 & 2.23 &            \\
101 & MWISP G24.700$-$0.124 & 107.86 & 2.84 & 85  & 130 & 101 & 26  & 5.15 & 4.08 & 15.8 & 21.7 & 1.1 & 3.0 & 3.3 & 2.2  & 2.3 & 3.8 & 0.16 & 2.84 &            \\
102 & MWISP G24.153$+$0.167 & 107.36 & 1.56 & 163 & 298 & 203 & -12 & 6.20 & 3.56 & 12.2 & 21.1 & 3.2 & 3.2 & 3.2 & 1.1  & 1.7 & 2.7 & 0.14 & 1.55 &            \\
103 & MWISP G24.923$+$0.201 & 96.75  & 1.07 & 110 & 111 & 110 & -20 & 5.77 & 3.80 & 16.6 & 21.4 & 1.4 & 2.8 & 2.5 & 0.5  & 2.1 & 3.5 & 0.16 & 1.06 &            \\
104 & MWISP G24.360$+$0.057 & 119.31 & 1.59 & 137 & 222 & 165 & 65  & 7.32 & 3.36 & 13.1 & 21.2 & 3.0 & 3.2 & 3.2 & 1.0  & 1.8 & 2.8 & 0.14 & 1.58 &            \\
105 & MWISP G24.722$+$0.115 & 109.18 & 2.64 & 99  & 105 & 102 & 121 & 6.31 & 3.58 & 15.7 & 21.6 & 1.4 & 3.0 & 3.3 & 2.1  & 2.2 & 3.6 & 0.16 & 2.64 &            \\
106 & MWISP G24.483$+$0.501 & 98.41  & 1.81 & 95  & 142 & 112 & 117 & 5.52 & 3.87 & 13.6 & 21.4 & 1.4 & 2.8 & 3.0 & 1.5  & 2.0 & 3.4 & 0.15 & 1.80 &            \\
107 & MWISP G24.491$-$0.009 & 109.02 & 1.80 & 87  & 100 & 93  & 68  & 6.20 & 3.59 & 14.1 & 21.6 & 1.2 & 2.9 & 2.9 & 1.1  & 2.2 & 3.7 & 0.15 & 1.79 &            \\
108 & MWISP G24.384$+$0.056 & 99.22  & 1.32 & 106 & 146 & 121 & 136 & 5.73 & 3.77 & 16.5 & 21.4 & 1.6 & 2.9 & 2.8 & 0.7  & 2.0 & 3.4 & 0.16 & 1.31 &            \\
109 & MWISP G24.522$-$0.061 & 82.97  & 1.75 & 116 & 151 & 130 & 23  & 5.20 & 4.04 & 14.7 & 21.2 & 1.5 & 2.6 & 3.0 & 2.3  & 1.8 & 3.1 & 0.15 & 1.74 &            \\
110 & MWISP G24.395$+$0.482 & 101.88 & 1.51 & 101 & 169 & 123 & 156 & 5.61 & 3.82 & 13.1 & 21.1 & 1.6 & 2.6 & 2.9 & 1.8  & 1.7 & 3.0 & 0.14 & 1.50 &            \\
111 & MWISP G24.666$-$0.274 & 96.41  & 1.36 & 117 & 221 & 147 & 31  & 5.58 & 3.86 & 10.9 & 20.9 & 2.1 & 2.6 & 2.9 & 1.9  & 1.5 & 2.7 & 0.13 & 1.35 &            \\
112 & MWISP G24.444$+$0.470 & 100.38 & 1.51 & 107 & 302 & 142 & 96  & 5.58 & 3.84 & 11.4 & 21.1 & 2.3 & 2.9 & 3.0 & 1.5  & 1.6 & 2.8 & 0.13 & 1.50 &            \\
113 & MWISP G24.548$-$0.245 & 99.39  & 1.68 & 52  & 65  & 57  & 29  & 5.70 & 3.79 & 12.9 & 21.2 & 0.4 & 2.0 & 2.3 & 2.1  & 2.4 & 4.4 & 0.14 & 1.67 &            \\
114 & MWISP G24.301$+$0.088 & 111.02 & 1.65 & 86  & 195 & 111 & 106 & 7.26 & 3.36 & 11.0 & 21.0 & 2.1 & 2.7 & 3.1 & 2.3  & 1.6 & 2.8 & 0.13 & 1.64 &            \\
115 & MWISP G24.345$+$0.157 & 113.99 & 1.08 & 134 & 188 & 154 & 6   & 7.17 & 3.37 & 10.5 & 20.8 & 2.6 & 2.7 & 2.8 & 1.2  & 1.4 & 2.5 & 0.13 & 1.07 &            \\
116 & MWISP G24.433$+$0.165 & 118.48 & 1.66 & 82  & 129 & 98  & 72  & 7.25 & 3.38 & 13.9 & 21.5 & 1.6 & 3.0 & 3.0 & 0.9  & 2.1 & 3.5 & 0.15 & 1.65 &            \\
117 & MWISP G24.420$+$0.241 & 114.00 & 1.81 & 138 & 319 & 179 & 120 & 6.85 & 3.42 & 10.5 & 21.0 & 3.4 & 3.0 & 3.4 & 2.1  & 1.5 & 2.5 & 0.13 & 1.81 &            \\
118 & MWISP G24.568$-$0.282 & 94.59  & 1.69 & 82  & 164 & 103 & -14 & 5.41 & 3.94 & 12.3 & 21.3 & 1.4 & 2.7 & 2.9 & 1.6  & 1.9 & 3.3 & 0.14 & 1.68 &            \\
119 & MWISP G24.466$+$0.224 & 117.82 & 1.71 & 73  & 153 & 93  & 12  & 7.19 & 3.38 & 8.6  & 20.9 & 1.6 & 2.4 & 3.0 & 3.7  & 1.5 & 2.9 & 0.12 & 1.71 &            \\
120 & MWISP G24.236$+$0.054 & 97.90  & 2.01 & 91  & 162 & 113 & 111 & 5.59 & 3.82 & 13.9 & 21.5 & 1.5 & 2.9 & 3.1 & 1.6  & 2.1 & 3.4 & 0.15 & 2.00 &            \\
121 & MWISP G24.435$-$0.033 & 107.51 & 1.54 & 126 & 183 & 147 & 154 & 5.07 & 4.11 & 13.5 & 21.4 & 1.8 & 3.0 & 2.9 & 0.9  & 2.0 & 3.3 & 0.15 & 1.53 &            \\
122 & MWISP G24.558$+$0.282 & 105.54 & 1.61 & 142 & 185 & 159 & 37  & 5.72 & 3.79 & 8.7  & 20.7 & 2.1 & 2.5 & 3.1 & 4.1  & 1.3 & 2.5 & 0.12 & 1.61 &            \\
123 & MWISP G24.835$-$0.144 & 89.30  & 1.46 & 163 & 202 & 179 & -7  & 5.34 & 3.99 & 12.7 & 21.4 & 2.3 & 3.1 & 3.0 & 0.7  & 1.9 & 3.1 & 0.14 & 1.45 &            \\
124 & MWISP G24.153$-$0.067 & 78.94  & 1.15 & 134 & 154 & 143 & 10  & 5.09 & 4.08 & 9.6  & 20.9 & 1.7 & 2.4 & 2.7 & 1.8  & 1.5 & 2.8 & 0.12 & 1.14 &            \\
125 & MWISP G24.325$-$0.001 & 116.32 & 2.62 & 129 & 173 & 146 & -22 & 7.30 & 3.36 & 18.0 & 21.9 & 2.5 & 3.7 & 3.6 & 0.7  & 2.4 & 3.6 & 0.17 & 2.61 & \checkmark \\
126 & MWISP G24.577$-$0.260 & 97.39  & 1.96 & 71  & 112 & 85  & 47  & 5.61 & 3.84 & 13.7 & 21.4 & 1.0 & 2.5 & 2.9 & 2.3  & 2.1 & 3.6 & 0.15 & 1.95 &            \\
127 & MWISP G24.395$-$0.007 & 115.15 & 2.91 & 173 & 252 & 201 & 53  & 7.24 & 3.37 & 15.8 & 21.6 & 3.5 & 3.8 & 3.8 & 1.1  & 2.2 & 3.2 & 0.16 & 2.91 &            \\
128 & MWISP G24.647$+$0.464 & 109.84 & 1.38 & 98  & 127 & 110 & 7   & 6.03 & 3.67 & 16.0 & 21.5 & 1.5 & 2.9 & 2.8 & 0.7  & 2.1 & 3.5 & 0.16 & 1.37 &            \\
129 & MWISP G24.723$-$0.265 & 93.75  & 2.18 & 143 & 223 & 171 & 49  & 5.45 & 3.93 & 14.2 & 21.4 & 2.3 & 3.1 & 3.4 & 1.6  & 1.9 & 3.1 & 0.15 & 2.17 &            \\
130 & MWISP G24.464$+$0.493 & 105.53 & 1.50 & 94  & 121 & 105 & 83  & 5.84 & 3.73 & 13.2 & 21.2 & 1.3 & 2.6 & 2.8 & 1.6  & 1.8 & 3.3 & 0.14 & 1.49 &            \\
131 & MWISP G24.947$+$0.213 & 98.70  & 1.18 & 110 & 167 & 130 & 22  & 5.82 & 3.78 & 19.9 & 21.7 & 1.8 & 3.3 & 2.7 & 0.3  & 2.3 & 3.6 & 0.18 & 1.17 &            \\
132 & MWISP G24.565$+$0.336 & 111.01 & 1.59 & 92  & 235 & 122 & -25 & 6.53 & 3.50 & 13.8 & 21.3 & 2.2 & 3.1 & 3.1 & 1.0  & 1.9 & 3.1 & 0.15 & 1.58 &            \\
133 & MWISP G24.365$+$0.070 & 112.35 & 1.72 & 67  & 91  & 77  & 59  & 6.91 & 3.40 & 11.3 & 21.1 & 1.0 & 2.3 & 2.8 & 2.8  & 1.9 & 3.4 & 0.13 & 1.71 &            \\
134 & MWISP G24.717$+$0.477 & 112.99 & 1.53 & 156 & 171 & 163 & 104 & 6.21 & 3.61 & 36.8 & 22.2 & 2.3 & 4.0 & 3.1 & 0.1  & 2.8 & 4.0 & 0.24 & 1.51 & \checkmark \\
135 & MWISP G24.215$-$0.055 & 91.42  & 2.42 & 98  & 119 & 107 & 92  & 5.27 & 3.98 & 11.0 & 21.2 & 1.2 & 2.5 & 3.2 & 4.4  & 1.9 & 3.3 & 0.13 & 2.42 &            \\
136 & MWISP G24.364$+$0.133 & 113.18 & 1.77 & 215 & 290 & 244 & 101 & 6.94 & 3.40 & 13.4 & 21.2 & 4.1 & 3.5 & 3.4 & 0.9  & 1.8 & 2.7 & 0.15 & 1.76 &            \\
137 & MWISP G25.030$+$0.045 & 106.52 & 1.33 & 109 & 169 & 130 & -21 & 6.06 & 3.69 & 14.6 & 21.4 & 1.8 & 3.0 & 2.8 & 0.7  & 2.0 & 3.2 & 0.15 & 1.32 &            \\
138 & MWISP G24.145$+$0.130 & 113.51 & 1.19 & 94  & 161 & 115 & 12  & 7.29 & 3.34 & 10.6 & 20.8 & 2.0 & 2.5 & 2.8 & 2.0  & 1.4 & 2.6 & 0.13 & 1.18 &            \\
139 & MWISP G24.301$-$0.150 & 100.72 & 2.69 & 59  & 80  & 67  & -20 & 5.72 & 3.76 & 10.3 & 21.2 & 0.6 & 2.2 & 3.0 & 6.7  & 2.0 & 3.8 & 0.13 & 2.69 &            \\
140 & MWISP G24.258$+$0.048 & 112.33 & 2.09 & 138 & 240 & 170 & 14  & 7.24 & 3.35 & 13.0 & 21.2 & 3.1 & 3.2 & 3.4 & 1.7  & 1.8 & 2.8 & 0.14 & 2.09 &            \\
141 & MWISP G24.341$+$0.283 & 110.19 & 1.45 & 73  & 94  & 81  & 120 & 6.30 & 3.54 & 11.7 & 21.1 & 1.0 & 2.3 & 2.6 & 2.4  & 1.8 & 3.3 & 0.14 & 1.44 &            \\
142 & MWISP G24.652$-$0.182 & 108.70 & 2.00 & 89  & 129 & 104 & 85  & 6.26 & 3.59 & 9.5  & 20.9 & 1.4 & 2.3 & 3.1 & 5.4  & 1.5 & 2.9 & 0.12 & 2.00 &            \\
143 & MWISP G24.616$-$0.103 & 82.29  & 1.94 & 96  & 139 & 111 & 75  & 5.20 & 4.05 & 9.8  & 21.1 & 1.3 & 2.4 & 3.0 & 4.0  & 1.7 & 3.1 & 0.12 & 1.94 &            \\
144 & MWISP G24.620$-$0.393 & 113.98 & 1.71 & 117 & 185 & 139 & 121 & 6.68 & 3.47 & 5.9  & 20.5 & 2.2 & 2.3 & 3.1 & 7.0  & 1.1 & 2.3 & 0.10 & 1.71 &            \\
145 & MWISP G24.509$+$0.259 & 119.48 & 2.21 & 68  & 110 & 82  & 30  & 6.99 & 3.41 & 8.4  & 20.9 & 1.2 & 2.2 & 3.1 & 7.3  & 1.6 & 3.0 & 0.11 & 2.21 &            \\
146 & MWISP G24.415$+$0.291 & 111.01 & 1.66 & 87  & 250 & 116 & 123 & 6.33 & 3.54 & 11.6 & 21.1 & 2.1 & 2.8 & 3.1 & 1.8  & 1.7 & 2.9 & 0.14 & 1.65 &            \\
147 & MWISP G24.894$+$0.219 & 97.56  & 1.46 & 105 & 105 & 105 & 36  & 5.78 & 3.79 & 14.9 & 21.4 & 1.3 & 2.8 & 2.8 & 0.9  & 2.1 & 3.5 & 0.15 & 1.45 &            \\
148 & MWISP G24.332$+$0.106 & 102.20 & 1.36 & 54  & 74  & 62  & 48  & 5.83 & 3.72 & 11.3 & 21.1 & 0.5 & 2.0 & 2.3 & 2.0  & 2.1 & 3.9 & 0.13 & 1.35 &            \\
149 & MWISP G24.326$+$0.300 & 114.17 & 1.04 & 74  & 166 & 96  & 78  & 6.71 & 3.43 & 11.5 & 20.9 & 1.6 & 2.4 & 2.6 & 1.5  & 1.5 & 2.8 & 0.13 & 1.03 &            \\
150 & MWISP G24.525$+$0.343 & 103.54 & 1.99 & 99  & 194 & 125 & 145 & 5.77 & 3.76 & 9.6  & 21.0 & 1.8 & 2.5 & 3.2 & 4.3  & 1.5 & 2.8 & 0.12 & 1.99 &            \\
151 & MWISP G24.268$-$0.074 & 88.92  & 1.48 & 87  & 177 & 111 & 71  & 5.21 & 4.02 & 10.6 & 21.0 & 1.4 & 2.4 & 2.8 & 2.5  & 1.6 & 3.0 & 0.13 & 1.47 &            \\
152 & MWISP G25.020$+$0.003 & 105.83 & 1.53 & 113 & 210 & 141 & 18  & 6.04 & 3.70 & 13.7 & 21.2 & 2.1 & 2.9 & 3.0 & 1.4  & 1.7 & 2.9 & 0.15 & 1.52 &            \\
153 & MWISP G24.327$+$0.198 & 110.69 & 1.79 & 160 & 202 & 177 & 87  & 6.77 & 3.42 & 11.3 & 21.1 & 2.8 & 3.1 & 3.3 & 1.5  & 1.7 & 2.8 & 0.13 & 1.79 &            \\
154 & MWISP G24.599$+$0.479 & 107.86 & 1.07 & 78  & 102 & 87  & 145 & 5.92 & 3.71 & 13.1 & 21.1 & 1.0 & 2.3 & 2.4 & 1.2  & 1.8 & 3.3 & 0.14 & 1.06 &            \\
155 & MWISP G24.439$-$0.311 & 95.73  & 2.00 & 83  & 98  & 89  & -7  & 5.39 & 3.94 & 14.3 & 21.5 & 1.0 & 2.6 & 2.9 & 1.8  & 2.2 & 3.7 & 0.15 & 1.99 &            \\
156 & MWISP G24.507$+$0.011 & 106.17 & 1.56 & 156 & 250 & 187 & 111 & 5.77 & 3.76 & 14.4 & 21.4 & 2.7 & 3.3 & 3.1 & 0.7  & 1.9 & 3.0 & 0.15 & 1.55 &            \\
157 & MWISP G24.348$+$0.226 & 87.94  & 2.01 & 102 & 103 & 103 & -6  & 5.22 & 4.02 & 10.4 & 21.1 & 1.1 & 2.3 & 3.0 & 4.6  & 1.7 & 3.2 & 0.13 & 2.01 &            \\
158 & MWISP G24.323$+$0.091 & 116.82 & 2.13 & 123 & 235 & 154 & 158 & 7.29 & 3.36 & 11.0 & 21.3 & 2.9 & 3.3 & 3.4 & 1.4  & 1.9 & 3.0 & 0.13 & 2.13 &            \\
159 & MWISP G24.245$+$0.225 & 114.99 & 1.10 & 116 & 230 & 147 & 139 & 7.23 & 3.35 & 11.4 & 21.1 & 2.7 & 3.1 & 2.8 & 0.6  & 1.7 & 2.8 & 0.13 & 1.09 &            \\
160 & MWISP G24.534$+$0.297 & 108.85 & 3.23 & 132 & 166 & 146 & 24  & 6.64 & 3.47 & 8.6  & 21.2 & 2.2 & 2.9 & 3.7 & 6.0  & 1.7 & 2.9 & 0.12 & 3.23 &            \\
161 & MWISP G24.256$-$0.419 & 91.41  & 1.37 & 84  & 165 & 106 & 15  & 5.02 & 4.13 & 5.1  & 20.4 & 1.3 & 1.8 & 2.7 & 8.7  & 1.0 & 2.5 & 0.09 & 1.37 &            \\
162 & MWISP G24.440$-$0.211 & 98.38  & 1.95 & 82  & 82  & 82  & 7   & 5.63 & 3.82 & 14.0 & 21.3 & 0.9 & 2.4 & 2.8 & 2.6  & 2.1 & 3.7 & 0.15 & 1.94 &            \\
163 & MWISP G24.468$+$0.427 & 100.88 & 1.45 & 103 & 181 & 127 & 24  & 5.63 & 3.82 & 9.6  & 20.9 & 1.7 & 2.5 & 2.9 & 2.5  & 1.5 & 2.8 & 0.12 & 1.44 &            \\
164 & MWISP G24.805$-$0.003 & 105.54 & 1.49 & 116 & 142 & 127 & 62  & 6.03 & 3.68 & 16.6 & 21.5 & 1.7 & 3.1 & 2.9 & 0.6  & 2.1 & 3.4 & 0.16 & 1.48 &            \\
165 & MWISP G24.297$+$0.210 & 113.99 & 1.09 & 114 & 204 & 141 & 81  & 7.19 & 3.36 & 12.0 & 21.2 & 2.5 & 3.1 & 2.8 & 0.5  & 1.8 & 2.9 & 0.14 & 1.08 &            \\
166 & MWISP G24.291$+$0.332 & 114.16 & 1.41 & 92  & 185 & 117 & 25  & 6.69 & 3.43 & 10.9 & 21.0 & 2.0 & 2.6 & 2.9 & 1.8  & 1.6 & 2.8 & 0.13 & 1.40 &            \\
167 & MWISP G24.476$-$0.210 & 96.74  & 1.58 & 69  & 131 & 86  & 1   & 5.56 & 3.85 & 13.6 & 21.2 & 1.1 & 2.4 & 2.8 & 2.0  & 1.9 & 3.4 & 0.15 & 1.57 &            \\
168 & MWISP G24.318$+$0.250 & 111.52 & 0.68 & 100 & 145 & 116 & 42  & 7.11 & 3.37 & 12.2 & 20.8 & 1.9 & 2.4 & 2.3 & 0.7  & 1.4 & 2.6 & 0.14 & 0.67 &            \\
169 & MWISP G24.442$+$0.373 & 115.33 & 1.96 & 102 & 260 & 134 & 112 & 6.65 & 3.46 & 11.3 & 21.3 & 2.5 & 3.2 & 3.3 & 1.4  & 1.9 & 3.0 & 0.13 & 1.96 &            \\
170 & MWISP G24.167$+$0.399 & 96.23  & 1.72 & 59  & 176 & 80  & -9  & 5.33 & 3.95 & 7.7  & 20.8 & 1.1 & 2.0 & 2.9 & 7.1  & 1.4 & 2.9 & 0.11 & 1.72 &            \\
171 & MWISP G24.444$+$0.049 & 99.20  & 1.01 & 98  & 98  & 98  & 46  & 5.76 & 3.76 & 22.2 & 21.5 & 1.2 & 2.8 & 2.4 & 0.4  & 2.2 & 3.7 & 0.19 & 0.99 &            \\
172 & MWISP G24.668$-$0.365 & 111.85 & 1.80 & 75  & 158 & 96  & -23 & 7.31 & 3.40 & 9.4  & 20.9 & 1.7 & 2.5 & 3.1 & 3.7  & 1.5 & 2.8 & 0.12 & 1.80 &            \\
173 & MWISP G24.467$-$0.061 & 84.61  & 1.06 & 67  & 124 & 83  & 39  & 5.21 & 4.03 & 8.9  & 20.6 & 1.0 & 1.7 & 2.3 & 4.3  & 1.3 & 2.8 & 0.12 & 1.05 &            \\
174 & MWISP G24.441$+$0.257 & 115.33 & 0.89 & 95  & 112 & 102 & 134 & 7.12 & 3.39 & 10.2 & 20.8 & 1.5 & 2.3 & 2.4 & 1.4  & 1.4 & 2.7 & 0.13 & 0.88 &            \\
175 & MWISP G24.951$-$0.120 & 79.60  & 1.13 & 114 & 313 & 152 & 158 & 5.29 & 4.03 & 9.3  & 20.9 & 2.3 & 2.7 & 2.8 & 1.2  & 1.5 & 2.6 & 0.12 & 1.12 &            \\
176 & MWISP G24.360$+$0.209 & 115.49 & 1.28 & 137 & 226 & 165 & 98  & 7.20 & 3.37 & 9.7  & 20.8 & 2.9 & 2.8 & 3.0 & 1.6  & 1.4 & 2.4 & 0.12 & 1.27 &            \\
177 & MWISP G24.546$+$0.102 & 114.17 & 1.33 & 82  & 147 & 101 & 2   & 6.92 & 3.42 & 12.5 & 21.0 & 1.6 & 2.6 & 2.8 & 1.6  & 1.7 & 3.0 & 0.14 & 1.32 &            \\
178 & MWISP G24.286$+$0.108 & 113.34 & 1.83 & 122 & 203 & 148 & 40  & 7.21 & 3.36 & 10.4 & 21.1 & 2.6 & 3.0 & 3.3 & 1.8  & 1.7 & 2.8 & 0.13 & 1.83 &            \\
179 & MWISP G24.574$-$0.217 & 98.39  & 1.46 & 104 & 165 & 124 & 1   & 5.69 & 3.80 & 14.8 & 21.3 & 1.7 & 2.8 & 2.9 & 1.1  & 1.9 & 3.2 & 0.15 & 1.45 &            \\
180 & MWISP G24.167$-$0.017 & 99.56  & 1.57 & 72  & 72  & 72  & 85  & 5.64 & 3.79 & 13.5 & 21.4 & 0.7 & 2.4 & 2.6 & 1.5  & 2.2 & 3.9 & 0.15 & 1.56 &            \\
181 & MWISP G24.257$+$0.261 & 112.34 & 1.15 & 70  & 78  & 73  & 21  & 7.12 & 3.36 & 10.1 & 20.9 & 0.9 & 2.1 & 2.4 & 2.1  & 1.7 & 3.3 & 0.13 & 1.14 &            \\
182 & MWISP G24.360$-$0.145 & 78.80  & 1.78 & 92  & 111 & 100 & 2   & 5.12 & 4.08 & 15.3 & 21.6 & 1.1 & 2.8 & 2.9 & 1.2  & 2.2 & 3.7 & 0.16 & 1.77 &            \\
183 & MWISP G24.502$+$0.365 & 107.36 & 1.49 & 144 & 189 & 162 & 20  & 6.57 & 3.48 & 10.1 & 20.9 & 2.5 & 2.7 & 3.1 & 2.1  & 1.4 & 2.6 & 0.13 & 1.48 &            \\
184 & MWISP G24.374$+$0.308 & 112.17 & 0.91 & 76  & 101 & 86  & -94 & 7.00 & 3.39 & 11.1 & 20.9 & 1.2 & 2.2 & 2.3 & 1.2  & 1.6 & 3.0 & 0.13 & 0.90 &            \\
185 & MWISP G24.667$-$0.186 & 79.62  & 1.57 & 91  & 213 & 119 & -10 & 5.17 & 4.07 & 14.3 & 21.3 & 1.6 & 2.8 & 2.9 & 1.4  & 1.9 & 3.2 & 0.15 & 1.56 &            \\
186 & MWISP G24.656$-$0.220 & 112.01 & 3.49 & 101 & 152 & 119 & 97  & 6.60 & 3.49 & 19.4 & 22.0 & 1.8 & 3.6 & 3.7 & 1.1  & 2.6 & 3.9 & 0.17 & 3.49 & \checkmark \\
187 & MWISP G24.403$+$0.021 & 109.69 & 1.89 & 61  & 172 & 81  & 40  & 6.17 & 3.59 & 18.1 & 21.6 & 1.3 & 3.0 & 3.0 & 1.0  & 2.2 & 3.7 & 0.17 & 1.88 &            \\
188 & MWISP G24.170$-$0.119 & 79.30  & 0.93 & 84  & 152 & 104 & 46  & 5.08 & 4.08 & 9.2  & 20.6 & 1.2 & 1.9 & 2.4 & 3.0  & 1.2 & 2.6 & 0.12 & 0.92 &            \\
189 & MWISP G24.820$-$0.148 & 80.13  & 1.62 & 109 & 177 & 131 & 115 & 5.25 & 4.04 & 11.8 & 21.3 & 1.6 & 2.8 & 3.0 & 1.3  & 1.9 & 3.2 & 0.14 & 1.61 &            \\
190 & MWISP G24.831$-$0.328 & 93.92  & 1.84 & 102 & 304 & 137 & 33  & 5.44 & 3.94 & 10.9 & 21.1 & 2.2 & 2.8 & 3.2 & 2.5  & 1.6 & 2.8 & 0.13 & 1.84 &            \\
191 & MWISP G24.564$-$0.147 & 96.41  & 1.41 & 77  & 200 & 102 & 33  & 5.63 & 3.83 & 14.2 & 21.2 & 1.5 & 2.6 & 2.8 & 1.5  & 1.8 & 3.1 & 0.15 & 1.40 &            \\
192 & MWISP G24.332$+$0.209 & 112.67 & 1.79 & 131 & 302 & 170 & 97  & 6.96 & 3.39 & 11.4 & 21.1 & 3.2 & 3.2 & 3.3 & 1.4  & 1.7 & 2.7 & 0.13 & 1.78 &            \\
193 & MWISP G24.483$-$0.269 & 98.23  & 1.51 & 72  & 157 & 92  & 120 & 5.60 & 3.84 & 16.8 & 21.5 & 1.3 & 2.8 & 2.8 & 1.0  & 2.1 & 3.5 & 0.16 & 1.50 &            \\
194 & MWISP G24.774$+$0.120 & 108.03 & 1.39 & 64  & 133 & 82  & 51  & 5.51 & 3.90 & 17.6 & 21.6 & 1.0 & 2.8 & 2.6 & 0.6  & 2.3 & 3.8 & 0.17 & 1.38 &            \\
195 & MWISP G24.157$+$0.073 & 107.69 & 1.72 & 77  & 132 & 94  & 63  & 6.33 & 3.51 & 13.5 & 21.3 & 1.3 & 2.7 & 2.9 & 1.8  & 1.9 & 3.3 & 0.15 & 1.71 &            \\
196 & MWISP G24.586$-$0.115 & 97.06  & 1.62 & 84  & 84  & 84  & 95  & 5.69 & 3.80 & 16.0 & 21.4 & 0.9 & 2.5 & 2.7 & 1.5  & 2.1 & 3.7 & 0.16 & 1.61 &            \\
197 & MWISP G24.423$+$0.358 & 111.35 & 1.58 & 91  & 114 & 101 & 100 & 5.96 & 3.67 & 8.7  & 20.9 & 1.3 & 2.2 & 2.8 & 3.8  & 1.5 & 3.0 & 0.12 & 1.58 &            \\
198 & MWISP G24.326$+$0.143 & 109.85 & 1.38 & 73  & 190 & 96  & 27  & 6.00 & 3.65 & 10.0 & 20.9 & 1.5 & 2.4 & 2.8 & 2.4  & 1.5 & 2.9 & 0.13 & 1.37 &            \\
199 & MWISP G24.172$+$0.256 & 113.00 & 1.62 & 108 & 177 & 130 & 176 & 7.27 & 3.34 & 10.6 & 20.9 & 2.3 & 2.7 & 3.1 & 2.4  & 1.5 & 2.7 & 0.13 & 1.61 &            \\
200 & MWISP G24.476$+$0.507 & 102.21 & 0.98 & 60  & 175 & 81  & -2  & 5.64 & 3.82 & 13.5 & 21.1 & 1.2 & 2.4 & 2.4 & 1.1  & 1.7 & 3.2 & 0.15 & 0.97 &            \\
201 & MWISP G24.561$+$0.340 & 106.55 & 1.63 & 100 & 200 & 126 & -15 & 5.91 & 3.71 & 14.7 & 21.5 & 1.9 & 3.1 & 3.0 & 0.8  & 2.1 & 3.3 & 0.15 & 1.62 &                          
\enddata
% \tablecomments{同表A1。}
\tablecomments{Same as Table \ref{appendix:the parameters of 12CO clumps}.}
\label{appendix:the parameters of 13CO clumps}
\end{deluxetable*}
\end{longrotatetable}

==> the_parameters_of_C18O_clumps.tex <==
\begin{longrotatetable}
\addtolength{\tabcolsep}{-1.5pt}
\begin{deluxetable*}{ccccccccccccccccccccc}
\tablecaption{The parameters of C$^{18}$O clumps}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{Number} & \colhead{Source} & \colhead{$V_{\text{lsr}}$} & \colhead{$\Delta v$} & \colhead{$\theta_{\text{a}}$} & \colhead{$\theta_{\text{b}}$} & \colhead{$\theta_{\text{fwhm}}$} & \colhead{P.A.} & \colhead{Distance} & \colhead{$R_{\text{GC}}$} & \colhead{$T_{\text{ex}}$} & \colhead{log($N_{\text{H$_2$}}$)} & \colhead{$R_{\text{eff}}$} & \colhead{log($M_{\text{clump}}$)} & \colhead{log($M_{\text{vir}}$)} & \colhead{$\alpha_{\text{vir}}$} & \colhead{log($\Sigma$)} & \colhead{log($n_{\text{H$_2$}}$)} & \colhead{$\Delta v_{\text{th}}$} & \colhead{$\Delta v_{\text{nth}}$} & \colhead{Potential} \\
\colhead{} & \colhead{} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{($\arcsec$)} & \colhead{($\arcsec$)} & \colhead{($\arcsec$)} & \colhead{($\arcdeg$)} & \colhead{(kpc)} & \colhead{(kpc)} & \colhead{(K)} & \colhead{(cm$^{-2}$)} & \colhead{(pc)} & \colhead{($M_{\sun}$)} & \colhead{($M_{\sun}$)} & \colhead{} & \colhead{($M_{\sun}$ pc$^{-2}$)} & \colhead{(cm$^{-3}$)} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{}
\decimalcolnumbers
}
\startdata
1   & MWISP G24.672$-$0.152 & 112.34 & 2.05 & 65  & 145 & 83  & 111 & 6.69 & 3.48 & 14.0 & 21.7 & 1.3 & 3.1 & 3.1 & 0.9 & 2.3 & 3.8 & 0.15 & 2.04 &            \\
2   & MWISP G24.785$+$0.088 & 109.01 & 1.82 & 110 & 158 & 128 & 122 & 5.28 & 4.02 & 18.7 & 22.0 & 1.6 & 3.5 & 3.0 & 0.4 & 2.6 & 3.9 & 0.17 & 1.81 & \checkmark \\
3   & MWISP G24.475$+$0.479 & 102.84 & 1.38 & 81  & 150 & 101 & 87  & 5.65 & 3.81 & 13.8 & 21.7 & 1.3 & 3.1 & 2.7 & 0.4 & 2.3 & 3.8 & 0.15 & 1.37 &            \\
4   & MWISP G24.788$+$0.095 & 110.67 & 1.53 & 123 & 146 & 133 & 122 & 6.46 & 3.54 & 17.0 & 21.9 & 1.9 & 3.5 & 3.0 & 0.3 & 2.5 & 3.7 & 0.16 & 1.52 & \checkmark \\
5   & MWISP G24.491$-$0.043 & 110.50 & 1.97 & 94  & 105 & 99  & 43  & 6.68 & 3.46 & 10.2 & 21.4 & 1.4 & 2.8 & 3.1 & 1.9 & 2.0 & 3.4 & 0.12 & 1.97 &            \\
6   & MWISP G24.555$+$0.334 & 108.34 & 1.55 & 92  & 184 & 116 & 153 & 6.56 & 3.49 & 14.7 & 21.6 & 1.9 & 3.2 & 3.0 & 0.6 & 2.2 & 3.4 & 0.15 & 1.54 &            \\
7   & MWISP G24.540$-$0.283 & 96.83  & 1.30 & 85  & 85  & 85  & 81  & 5.54 & 3.87 & 12.1 & 21.4 & 0.9 & 2.5 & 2.5 & 1.0 & 2.1 & 3.7 & 0.14 & 1.29 &            \\
8   & MWISP G24.203$-$0.259 & 93.66  & 1.25 & 82  & 92  & 87  & 84  & 5.25 & 3.99 & 6.3  & 21.2 & 0.9 & 2.2 & 2.5 & 1.7 & 1.8 & 3.4 & 0.10 & 1.25 &            \\
9   & MWISP G24.457$+$0.191 & 119.17 & 1.75 & 83  & 150 & 103 & 35  & 7.23 & 3.38 & 10.6 & 21.5 & 1.7 & 3.1 & 3.0 & 0.8 & 2.1 & 3.4 & 0.13 & 1.75 &            \\
10  & MWISP G24.742$+$0.151 & 107.18 & 1.14 & 67  & 110 & 81  & 129 & 6.05 & 3.67 & 17.0 & 21.6 & 1.0 & 2.8 & 2.4 & 0.4 & 2.3 & 3.8 & 0.16 & 1.13 &            \\
11  & MWISP G24.798$+$0.098 & 107.33 & 1.45 & 77  & 104 & 87  & 104 & 6.08 & 3.66 & 15.9 & 21.8 & 1.1 & 3.0 & 2.7 & 0.5 & 2.4 & 3.9 & 0.16 & 1.44 & \checkmark \\
12  & MWISP G24.410$+$0.111 & 110.01 & 1.40 & 71  & 164 & 93  & 75  & 6.11 & 3.61 & 14.3 & 21.9 & 1.4 & 3.3 & 2.8 & 0.3 & 2.5 & 3.9 & 0.15 & 1.39 & \checkmark \\
13  & MWISP G24.558$-$0.215 & 100.00 & 1.34 & 82  & 143 & 100 & 17  & 5.75 & 3.77 & 15.5 & 21.4 & 1.3 & 2.8 & 2.7 & 0.8 & 2.0 & 3.5 & 0.15 & 1.33 &            \\
14  & MWISP G24.488$+$0.464 & 103.99 & 0.91 & 93  & 173 & 116 & 45  & 5.68 & 3.80 & 12.4 & 21.4 & 1.6 & 2.9 & 2.4 & 0.4 & 2.0 & 3.3 & 0.14 & 0.90 &            \\
15  & MWISP G24.358$+$0.066 & 118.50 & 1.69 & 73  & 152 & 93  & -20 & 7.31 & 3.36 & 11.5 & 21.5 & 1.6 & 3.0 & 3.0 & 0.9 & 2.1 & 3.4 & 0.13 & 1.68 &            \\
16  & MWISP G24.651$-$0.176 & 112.83 & 1.67 & 64  & 141 & 83  & 80  & 6.81 & 3.45 & 12.4 & 21.3 & 1.3 & 2.7 & 2.9 & 1.4 & 2.0 & 3.4 & 0.14 & 1.66 &            \\
17  & MWISP G24.849$-$0.027 & 105.00 & 1.12 & 72  & 85  & 78  & -43 & 6.01 & 3.69 & 12.6 & 21.2 & 0.9 & 2.3 & 2.4 & 1.1 & 1.9 & 3.6 & 0.14 & 1.11 &            \\
18  & MWISP G24.366$+$0.273 & 111.67 & 1.24 & 79  & 110 & 91  & -5  & 7.05 & 3.38 & 13.0 & 21.4 & 1.3 & 2.8 & 2.6 & 0.7 & 2.1 & 3.5 & 0.14 & 1.23 &            \\
19  & MWISP G24.422$+$0.117 & 112.67 & 2.27 & 111 & 176 & 133 & 80  & 6.87 & 3.41 & 14.9 & 22.1 & 2.2 & 3.9 & 3.4 & 0.3 & 2.7 & 3.9 & 0.15 & 2.26 & \checkmark \\
20  & MWISP G24.550$-$0.243 & 98.84  & 1.76 & 80  & 80  & 80  & 72  & 5.68 & 3.80 & 14.8 & 21.5 & 0.8 & 2.6 & 2.7 & 1.5 & 2.2 & 3.8 & 0.15 & 1.75 &            \\
21  & MWISP G24.236$+$0.205 & 113.50 & 1.32 & 75  & 118 & 89  & 42  & 7.21 & 3.35 & 10.2 & 21.4 & 1.4 & 2.9 & 2.7 & 0.7 & 2.1 & 3.5 & 0.12 & 1.31 &            \\
22  & MWISP G24.541$+$0.498 & 109.66 & 0.82 & 54  & 81  & 64  & 98  & 6.04 & 3.65 & 10.9 & 21.1 & 0.6 & 2.1 & 1.9 & 0.7 & 2.0 & 3.8 & 0.13 & 0.81 &            \\
23  & MWISP G24.516$-$0.286 & 97.00  & 1.25 & 52  & 108 & 66  & 14  & 5.53 & 3.87 & 15.3 & 21.6 & 0.7 & 2.6 & 2.4 & 0.7 & 2.3 & 4.0 & 0.15 & 1.24 &            \\
24  & MWISP G24.568$+$0.336 & 109.84 & 0.98 & 82  & 134 & 99  & -1  & 6.30 & 3.57 & 13.8 & 21.3 & 1.4 & 2.7 & 2.4 & 0.5 & 2.0 & 3.4 & 0.15 & 0.97 &            \\
25  & MWISP G24.766$+$0.117 & 109.17 & 1.05 & 64  & 164 & 85  & 112 & 6.28 & 3.59 & 19.4 & 21.9 & 1.4 & 3.3 & 2.5 & 0.2 & 2.5 & 3.9 & 0.17 & 1.04 & \checkmark \\
26  & MWISP G24.211$+$0.243 & 113.67 & 1.06 & 103 & 170 & 125 & 27  & 7.31 & 3.34 & 9.8  & 21.2 & 2.2 & 3.0 & 2.7 & 0.5 & 1.8 & 3.0 & 0.12 & 1.05 &            \\
27  & MWISP G24.791$+$0.101 & 112.00 & 1.19 & 68  & 89  & 76  & 89  & 6.59 & 3.51 & 17.5 & 21.8 & 0.9 & 3.0 & 2.4 & 0.3 & 2.5 & 4.1 & 0.16 & 1.18 & \checkmark \\
28  & MWISP G25.001$+$0.001 & 105.67 & 0.44 & 52  & 99  & 65  & 6   & 6.03 & 3.70 & 14.8 & 21.0 & 0.7 & 2.0 & 1.5 & 0.3 & 1.8 & 3.5 & 0.15 & 0.41 &            \\
29  & MWISP G24.575$-$0.266 & 97.33  & 1.48 & 66  & 99  & 78  & 18  & 5.60 & 3.84 & 13.7 & 21.5 & 0.9 & 2.6 & 2.6 & 1.0 & 2.2 & 3.8 & 0.14 & 1.47 &            \\
30  & MWISP G24.216$+$0.118 & 102.34 & 1.41 & 88  & 89  & 89  & 80  & 5.68 & 3.77 & 11.6 & 21.5 & 1.0 & 2.6 & 2.6 & 1.0 & 2.1 & 3.7 & 0.13 & 1.40 &            \\
31  & MWISP G24.866$+$0.008 & 109.49 & 0.87 & 57  & 89  & 68  & 113 & 5.32 & 4.01 & 14.6 & 21.5 & 0.6 & 2.4 & 2.0 & 0.4 & 2.3 & 4.1 & 0.15 & 0.86 &            \\
32  & MWISP G24.234$+$0.050 & 98.17  & 1.24 & 76  & 106 & 87  & 109 & 5.60 & 3.81 & 13.9 & 21.5 & 1.0 & 2.6 & 2.5 & 0.7 & 2.1 & 3.7 & 0.15 & 1.23 &            \\
33  & MWISP G24.531$-$0.209 & 101.83 & 1.37 & 63  & 107 & 77  & 2   & 5.80 & 3.75 & 17.9 & 21.9 & 0.9 & 3.1 & 2.5 & 0.3 & 2.7 & 4.2 & 0.17 & 1.36 & \checkmark \\
34  & MWISP G24.500$+$0.051 & 98.66  & 1.07 & 76  & 110 & 89  & 140 & 5.76 & 3.76 & 13.8 & 21.1 & 1.1 & 2.4 & 2.4 & 1.1 & 1.8 & 3.3 & 0.15 & 1.06 &            \\
35  & MWISP G24.542$-$0.134 & 94.83  & 1.56 & 79  & 146 & 98  & 20  & 5.53 & 3.87 & 14.8 & 21.6 & 1.3 & 3.0 & 2.8 & 0.7 & 2.3 & 3.7 & 0.15 & 1.55 &            \\
36  & MWISP G24.200$-$0.059 & 89.17  & 1.18 & 73  & 73  & 73  & 105 & 5.20 & 4.02 & 9.7  & 21.5 & 0.7 & 2.4 & 2.3 & 0.7 & 2.3 & 4.0 & 0.12 & 1.17 &            \\
37  & MWISP G24.635$-$0.108 & 112.84 & 2.63 & 86  & 116 & 98  & 16  & 6.78 & 3.45 & 11.2 & 21.5 & 1.4 & 2.9 & 3.3 & 2.3 & 2.1 & 3.5 & 0.13 & 2.63 &            \\
38  & MWISP G24.366$+$0.090 & 116.50 & 1.40 & 88  & 175 & 111 & 51  & 7.27 & 3.37 & 11.4 & 21.4 & 2.0 & 3.1 & 2.9 & 0.7 & 2.0 & 3.2 & 0.13 & 1.39 &            \\
39  & MWISP G24.436$+$0.235 & 118.50 & 1.65 & 82  & 112 & 93  & 111 & 7.20 & 3.38 & 9.7  & 21.3 & 1.4 & 2.8 & 2.9 & 1.4 & 2.0 & 3.4 & 0.12 & 1.65 &            \\
40  & MWISP G24.436$-$0.274 & 95.83  & 1.09 & 61  & 139 & 79  & 30  & 5.43 & 3.91 & 12.2 & 21.3 & 1.0 & 2.4 & 2.4 & 0.9 & 1.9 & 3.5 & 0.14 & 1.08 &            \\
41  & MWISP G24.475$+$0.433 & 103.67 & 0.85 & 64  & 88  & 73  & 43  & 5.66 & 3.81 & 13.5 & 21.2 & 0.8 & 2.2 & 2.1 & 0.7 & 2.0 & 3.6 & 0.14 & 0.84 &            \\
42  & MWISP G24.317$+$0.136 & 112.01 & 1.59 & 61  & 124 & 78  & 3   & 6.88 & 3.40 & 11.7 & 21.4 & 1.2 & 2.8 & 2.8 & 1.1 & 2.1 & 3.6 & 0.13 & 1.58 &            \\
43  & MWISP G24.517$+$0.317 & 107.84 & 0.37 & 54  & 101 & 67  & 78  & 6.61 & 3.48 & 9.7  & 20.7 & 0.9 & 1.9 & 1.4 & 0.3 & 1.5 & 3.1 & 0.12 & 0.35 &            \\
44  & MWISP G24.458$+$0.506 & 100.83 & 1.11 & 61  & 174 & 81  & 29  & 5.60 & 3.83 & 12.8 & 21.3 & 1.2 & 2.6 & 2.5 & 0.8 & 1.9 & 3.4 & 0.14 & 1.10 &            \\
45  & MWISP G24.358$+$0.041 & 117.00 & 2.17 & 90  & 130 & 104 & 58  & 7.30 & 3.36 & 16.1 & 21.9 & 1.7 & 3.5 & 3.2 & 0.5 & 2.6 & 3.9 & 0.16 & 2.16 & \checkmark \\
46  & MWISP G24.463$+$0.260 & 119.50 & 1.29 & 66  & 143 & 84  & 132 & 7.02 & 3.40 & 9.8  & 21.3 & 1.4 & 2.8 & 2.7 & 0.8 & 2.0 & 3.4 & 0.12 & 1.28 &            \\
47  & MWISP G24.358$+$0.275 & 113.17 & 1.13 & 115 & 138 & 125 & 93  & 7.08 & 3.38 & 10.5 & 21.2 & 2.0 & 2.9 & 2.7 & 0.7 & 1.8 & 3.0 & 0.13 & 1.12 &            \\
48  & MWISP G24.656$-$0.175 & 110.67 & 1.78 & 79  & 88  & 83  & 87  & 6.51 & 3.52 & 13.6 & 21.6 & 1.0 & 2.8 & 2.8 & 1.0 & 2.3 & 3.8 & 0.14 & 1.77 &            \\
49  & MWISP G24.157$+$0.165 & 106.85 & 1.08 & 93  & 141 & 110 & -3  & 6.19 & 3.56 & 11.5 & 21.3 & 1.5 & 2.7 & 2.6 & 0.7 & 1.9 & 3.2 & 0.13 & 1.07 &            \\
50  & MWISP G24.734$+$0.109 & 110.33 & 1.12 & 65  & 110 & 79  & 1   & 6.45 & 3.54 & 16.7 & 21.4 & 1.1 & 2.7 & 2.4 & 0.6 & 2.1 & 3.6 & 0.16 & 1.11 &            \\
51  & MWISP G24.134$+$0.251 & 113.50 & 1.05 & 80  & 126 & 95  & -2  & 7.36 & 3.33 & 11.2 & 21.2 & 1.5 & 2.7 & 2.6 & 0.8 & 1.8 & 3.2 & 0.13 & 1.04 &            \\
52  & MWISP G24.842$+$0.033 & 106.17 & 1.28 & 67  & 124 & 83  & 48  & 6.05 & 3.68 & 16.0 & 21.8 & 1.1 & 3.1 & 2.6 & 0.3 & 2.5 & 4.0 & 0.16 & 1.27 & \checkmark \\
53  & MWISP G24.444$+$0.203 & 121.00 & 1.49 & 101 & 175 & 123 & 99  & 7.23 & 3.38 & 10.4 & 21.5 & 2.1 & 3.2 & 3.0 & 0.6 & 2.0 & 3.2 & 0.13 & 1.48 &            \\
54  & MWISP G24.483$+$0.467 & 101.83 & 1.08 & 53  & 105 & 67  & 53  & 5.48 & 3.89 & 12.6 & 21.5 & 0.7 & 2.5 & 2.2 & 0.6 & 2.2 & 3.9 & 0.14 & 1.07 &            \\
55  & MWISP G24.690$+$0.442 & 111.84 & 1.34 & 73  & 156 & 94  & 136 & 5.92 & 3.71 & 21.1 & 22.0 & 1.3 & 3.4 & 2.7 & 0.2 & 2.6 & 4.0 & 0.18 & 1.33 & \checkmark \\
56  & MWISP G24.781$-$0.026 & 109.00 & 1.48 & 72  & 135 & 89  & 30  & 5.32 & 4.00 & 16.7 & 21.7 & 1.1 & 2.9 & 2.7 & 0.7 & 2.3 & 3.8 & 0.16 & 1.47 &            \\
57  & MWISP G24.533$+$0.330 & 112.16 & 0.98 & 83  & 87  & 85  & 27  & 6.30 & 3.56 & 8.9  & 21.2 & 1.0 & 2.4 & 2.3 & 0.9 & 1.9 & 3.4 & 0.12 & 0.97 &            \\
58  & MWISP G24.548$+$0.484 & 102.67 & 1.03 & 76  & 139 & 94  & 128 & 5.66 & 3.81 & 9.7  & 21.2 & 1.2 & 2.5 & 2.4 & 0.9 & 1.8 & 3.3 & 0.12 & 1.02 &            \\
59  & MWISP G24.416$+$0.058 & 114.83 & 1.35 & 55  & 102 & 68  & 65  & 7.23 & 3.37 & 21.8 & 22.0 & 1.0 & 3.3 & 2.6 & 0.2 & 2.8 & 4.4 & 0.18 & 1.34 & \checkmark \\
60  & MWISP G24.350$+$0.123 & 118.00 & 1.24 & 82  & 109 & 92  & 60  & 7.29 & 3.36 & 11.6 & 21.4 & 1.4 & 2.9 & 2.7 & 0.6 & 2.1 & 3.5 & 0.13 & 1.23 &            \\
61  & MWISP G24.291$+$0.201 & 113.50 & 1.19 & 52  & 76  & 60  & -10 & 7.16 & 3.36 & 12.7 & 21.5 & 0.6 & 2.6 & 2.3 & 0.5 & 2.5 & 4.3 & 0.14 & 1.18 &            \\
62  & MWISP G24.198$+$0.407 & 96.00  & 1.45 & 74  & 97  & 83  & 133 & 5.33 & 3.95 & 9.1  & 21.4 & 0.9 & 2.5 & 2.6 & 1.2 & 2.1 & 3.7 & 0.12 & 1.45 &            \\
63  & MWISP G24.450$+$0.433 & 102.17 & 0.38 & 52  & 107 & 66  & -6  & 5.62 & 3.82 & 6.4  & 20.6 & 0.7 & 1.6 & 1.3 & 0.5 & 1.4 & 3.1 & 0.10 & 0.37 &            \\
64  & MWISP G24.858$+$0.034 & 109.33 & 0.64 & 51  & 107 & 65  & 61  & 5.32 & 4.01 & 14.8 & 21.5 & 0.7 & 2.4 & 1.8 & 0.2 & 2.3 & 4.0 & 0.15 & 0.62 &            \\
65  & MWISP G24.365$+$0.083 & 97.33  & 0.99 & 80  & 106 & 91  & -17 & 5.63 & 3.81 & 11.4 & 21.3 & 1.1 & 2.5 & 2.3 & 0.7 & 2.0 & 3.5 & 0.13 & 0.98 &            \\
66  & MWISP G24.808$+$0.035 & 107.50 & 1.02 & 59  & 130 & 76  & -11 & 6.10 & 3.66 & 18.2 & 21.7 & 1.1 & 2.9 & 2.4 & 0.3 & 2.4 & 3.9 & 0.17 & 1.01 &            \\
67  & MWISP G24.233$+$0.239 & 114.66 & 0.69 & 130 & 139 & 134 & 144 & 7.22 & 3.35 & 9.7  & 21.1 & 2.2 & 2.9 & 2.3 & 0.3 & 1.7 & 2.9 & 0.12 & 0.68 &            \\
68  & MWISP G24.642$+$0.376 & 109.84 & 1.07 & 85  & 86  & 85  & 105 & 6.70 & 3.47 & 13.5 & 21.4 & 1.1 & 2.7 & 2.4 & 0.5 & 2.1 & 3.6 & 0.14 & 1.06 &            \\
69  & MWISP G24.524$+$0.317 & 108.51 & 0.83 & 75  & 175 & 98  & 72  & 6.61 & 3.48 & 9.2  & 21.0 & 1.7 & 2.6 & 2.4 & 0.7 & 1.6 & 2.9 & 0.12 & 0.82 &            \\
70  & MWISP G24.941$+$0.184 & 97.67  & 0.97 & 70  & 170 & 92  & 43  & 5.80 & 3.79 & 17.1 & 21.7 & 1.4 & 3.1 & 2.4 & 0.2 & 2.3 & 3.7 & 0.16 & 0.96 &            \\
71  & MWISP G25.017$+$0.041 & 106.34 & 0.75 & 90  & 131 & 105 & -44 & 6.06 & 3.69 & 15.0 & 21.3 & 1.4 & 2.7 & 2.2 & 0.3 & 1.9 & 3.3 & 0.15 & 0.73 &            \\
72  & MWISP G24.166$+$0.398 & 94.50  & 1.53 & 73  & 173 & 95  & -12 & 5.26 & 3.98 & 8.3  & 21.4 & 1.3 & 2.7 & 2.8 & 1.3 & 2.0 & 3.4 & 0.11 & 1.53 &            \\
73  & MWISP G24.144$-$0.115 & 79.67  & 0.96 & 82  & 109 & 93  & 28  & 5.07 & 4.09 & 10.0 & 21.3 & 1.0 & 2.4 & 2.3 & 0.7 & 1.9 & 3.5 & 0.12 & 0.95 &            \\
74  & MWISP G24.517$-$0.066 & 83.83  & 1.39 & 79  & 89  & 84  & 67  & 5.21 & 4.04 & 15.2 & 21.3 & 0.8 & 2.4 & 2.5 & 1.5 & 2.0 & 3.6 & 0.15 & 1.38 &            \\
75  & MWISP G24.118$+$0.125 & 113.00 & 0.88 & 83  & 182 & 107 & 5   & 7.15 & 3.34 & 12.2 & 21.3 & 1.9 & 2.9 & 2.5 & 0.4 & 1.9 & 3.1 & 0.14 & 0.87 &            \\
76  & MWISP G24.350$+$0.016 & 118.17 & 1.17 & 65  & 97  & 76  & 41  & 7.32 & 3.36 & 17.8 & 21.8 & 1.1 & 3.1 & 2.5 & 0.3 & 2.5 & 4.0 & 0.16 & 1.16 & \checkmark \\
77  & MWISP G24.350$+$0.149 & 112.67 & 0.40 & 71  & 143 & 90  & 6   & 6.90 & 3.40 & 10.1 & 20.8 & 1.4 & 2.3 & 1.7 & 0.3 & 1.5 & 2.9 & 0.12 & 0.38 &            \\
78  & MWISP G24.340$+$0.259 & 105.50 & 1.44 & 69  & 158 & 90  & 19  & 6.78 & 3.42 & 11.3 & 21.5 & 1.5 & 2.9 & 2.8 & 0.7 & 2.1 & 3.5 & 0.13 & 1.43 &            \\
79  & MWISP G24.327$+$0.054 & 114.50 & 1.58 & 91  & 171 & 113 & 59  & 7.21 & 3.36 & 15.2 & 21.6 & 2.0 & 3.3 & 3.0 & 0.5 & 2.2 & 3.4 & 0.15 & 1.57 &            \\
80  & MWISP G24.191$+$0.056 & 109.17 & 1.40 & 71  & 192 & 94  & 25  & 7.08 & 3.36 & 12.9 & 21.5 & 1.8 & 3.1 & 2.9 & 0.6 & 2.1 & 3.4 & 0.14 & 1.39 &            \\
81  & MWISP G24.676$-$0.151 & 113.67 & 1.55 & 60  & 96  & 72  & 157 & 6.81 & 3.45 & 14.4 & 21.6 & 0.9 & 2.8 & 2.7 & 0.7 & 2.4 & 4.0 & 0.15 & 1.54 &            \\
82  & MWISP G24.524$+$0.349 & 107.34 & 0.90 & 103 & 147 & 119 & 20  & 6.08 & 3.64 & 11.9 & 21.2 & 1.6 & 2.7 & 2.4 & 0.5 & 1.8 & 3.1 & 0.13 & 0.89 &            \\
83  & MWISP G24.441$+$0.374 & 115.00 & 1.09 & 71  & 152 & 91  & 118 & 6.63 & 3.46 & 10.6 & 21.2 & 1.5 & 2.6 & 2.6 & 0.8 & 1.8 & 3.2 & 0.13 & 1.08 &            \\
84  & MWISP G24.484$+$0.157 & 118.67 & 1.24 & 55  & 68  & 60  & 129 & 7.24 & 3.38 & 12.5 & 21.2 & 0.6 & 2.3 & 2.3 & 1.0 & 2.2 & 4.0 & 0.14 & 1.23 &            \\
85  & MWISP G24.384$+$0.052 & 99.50  & 1.02 & 71  & 100 & 82  & 137 & 5.75 & 3.76 & 16.5 & 21.6 & 0.9 & 2.7 & 2.3 & 0.4 & 2.3 & 3.8 & 0.16 & 1.01 &            \\
86  & MWISP G24.510$-$0.217 & 100.66 & 1.13 & 55  & 121 & 71  & 127 & 5.75 & 3.77 & 12.6 & 21.3 & 0.9 & 2.4 & 2.4 & 1.0 & 2.0 & 3.6 & 0.14 & 1.12 &            \\
87  & MWISP G24.656$-$0.107 & 115.17 & 1.48 & 65  & 84  & 72  & 76  & 6.95 & 3.43 & 9.7  & 21.3 & 0.9 & 2.5 & 2.6 & 1.4 & 2.1 & 3.7 & 0.12 & 1.47 &            \\
88  & MWISP G24.839$-$0.027 & 103.50 & 0.99 & 61  & 84  & 70  & 2   & 5.95 & 3.72 & 13.4 & 21.2 & 0.7 & 2.2 & 2.2 & 0.9 & 2.0 & 3.7 & 0.14 & 0.98 &            \\
89  & MWISP G24.667$-$0.116 & 113.00 & 2.24 & 61  & 83  & 70  & 88  & 7.01 & 3.42 & 13.4 & 21.8 & 0.8 & 3.0 & 2.9 & 0.9 & 2.6 & 4.3 & 0.14 & 2.24 & \checkmark \\
90  & MWISP G24.410$+$0.101 & 114.50 & 1.18 & 56  & 111 & 70  & -4  & 7.21 & 3.37 & 15.4 & 22.0 & 1.0 & 3.2 & 2.5 & 0.2 & 2.7 & 4.2 & 0.15 & 1.17 & \checkmark \\
91  & MWISP G24.383$+$0.025 & 117.83 & 1.21 & 77  & 220 & 103 & 101 & 7.30 & 3.37 & 17.8 & 21.8 & 2.1 & 3.6 & 2.8 & 0.2 & 2.4 & 3.6 & 0.16 & 1.20 & \checkmark \\
92  & MWISP G25.010$+$0.008 & 105.17 & 0.49 & 92  & 123 & 104 & 18  & 6.02 & 3.71 & 13.0 & 21.0 & 1.4 & 2.4 & 1.8 & 0.3 & 1.6 & 3.1 & 0.14 & 0.47 &            \\
93  & MWISP G24.566$+$0.359 & 109.17 & 0.64 & 52  & 70  & 59  & -14 & 6.69 & 3.46 & 16.3 & 21.2 & 0.5 & 2.2 & 1.6 & 0.3 & 2.3 & 4.1 & 0.16 & 0.62 &            \\
94  & MWISP G24.307$+$0.099 & 113.34 & 1.13 & 62  & 159 & 82  & 16  & 7.21 & 3.36 & 10.3 & 21.2 & 1.5 & 2.7 & 2.6 & 0.9 & 1.8 & 3.2 & 0.13 & 1.12 &            \\
95  & MWISP G24.676$-$0.149 & 110.83 & 1.42 & 53  & 66  & 59  & 80  & 6.54 & 3.51 & 14.4 & 21.6 & 0.5 & 2.5 & 2.3 & 0.6 & 2.7 & 4.6 & 0.15 & 1.41 & \checkmark \\
96  & MWISP G24.416$+$0.475 & 102.67 & 0.34 & 62  & 94  & 73  & 101 & 5.64 & 3.81 & 16.1 & 21.1 & 0.8 & 2.1 & 1.3 & 0.1 & 1.8 & 3.5 & 0.16 & 0.30 &            \\
97  & MWISP G24.425$+$0.149 & 115.34 & 1.12 & 81  & 147 & 101 & 13  & 7.20 & 3.38 & 13.6 & 21.6 & 1.7 & 3.1 & 2.6 & 0.3 & 2.2 & 3.5 & 0.14 & 1.11 &            \\
98  & MWISP G24.541$-$0.251 & 97.00  & 1.21 & 57  & 78  & 65  & 70  & 5.58 & 3.85 & 14.4 & 21.6 & 0.6 & 2.5 & 2.3 & 0.6 & 2.4 & 4.2 & 0.15 & 1.20 &            \\
99  & MWISP G24.744$+$0.175 & 108.50 & 1.29 & 65  & 100 & 77  & 73  & 6.17 & 3.63 & 17.5 & 21.9 & 0.9 & 3.1 & 2.5 & 0.3 & 2.6 & 4.2 & 0.16 & 1.28 & \checkmark \\
100 & MWISP G24.800$-$0.097 & 80.83  & 1.14 & 87  & 112 & 97  & 69  & 5.27 & 4.03 & 9.9  & 21.2 & 1.1 & 2.4 & 2.5 & 1.1 & 1.9 & 3.4 & 0.12 & 1.13 &            \\
101 & MWISP G24.167$-$0.018 & 99.84  & 0.87 & 57  & 72  & 63  & 34  & 5.65 & 3.78 & 13.5 & 21.4 & 0.5 & 2.3 & 1.9 & 0.4 & 2.4 & 4.2 & 0.14 & 0.86 &            \\
102 & MWISP G24.446$+$0.183 & 116.83 & 1.14 & 89  & 204 & 116 & 89  & 7.21 & 3.38 & 13.0 & 21.4 & 2.2 & 3.1 & 2.8 & 0.5 & 1.9 & 3.1 & 0.14 & 1.13 &            \\
103 & MWISP G24.436$+$0.266 & 117.33 & 1.56 & 104 & 149 & 121 & 82  & 7.16 & 3.38 & 9.9  & 21.3 & 2.0 & 3.0 & 3.0 & 1.1 & 1.9 & 3.1 & 0.12 & 1.56 &            \\
104 & MWISP G24.400$+$0.158 & 113.50 & 1.12 & 72  & 128 & 89  & 98  & 6.92 & 3.40 & 12.7 & 21.3 & 1.4 & 2.7 & 2.6 & 0.7 & 1.9 & 3.4 & 0.14 & 1.11 &            \\
105 & MWISP G24.201$-$0.333 & 89.00  & 0.94 & 66  & 96  & 77  & 127 & 5.04 & 4.11 & 4.8  & 21.0 & 0.7 & 2.0 & 2.1 & 1.5 & 1.7 & 3.4 & 0.09 & 0.94 &            \\
106 & MWISP G24.508$-$0.108 & 94.84  & 1.35 & 79  & 118 & 93  & 68  & 5.52 & 3.88 & 12.2 & 21.4 & 1.1 & 2.6 & 2.6 & 1.1 & 2.0 & 3.5 & 0.14 & 1.34 &            \\
107 & MWISP G24.467$+$0.458 & 103.34 & 0.88 & 52  & 72  & 59  & 3   & 5.66 & 3.81 & 13.4 & 21.5 & 0.5 & 2.4 & 1.9 & 0.3 & 2.6 & 4.4 & 0.14 & 0.87 &            \\
108 & MWISP G25.018$+$0.050 & 107.33 & 0.57 & 66  & 116 & 81  & 13  & 6.09 & 3.68 & 14.8 & 21.4 & 1.1 & 2.6 & 1.9 & 0.2 & 2.1 & 3.6 & 0.15 & 0.55 &            \\
109 & MWISP G24.950$+$0.466 & 111.33 & 0.79 & 53  & 63  & 58  & 127 & 6.19 & 3.64 & 14.4 & 21.1 & 0.4 & 2.0 & 1.7 & 0.6 & 2.2 & 4.2 & 0.15 & 0.78 &            \\
110 & MWISP G24.333$+$0.217 & 112.67 & 0.73 & 53  & 138 & 70  & 38  & 6.96 & 3.39 & 11.9 & 21.1 & 1.2 & 2.5 & 2.1 & 0.4 & 1.8 & 3.3 & 0.13 & 0.72 &                          
\enddata
% \tablecomments{同表A1。}
\tablecomments{Same as Table \ref{appendix:the parameters of 12CO clumps}.}
\label{appendix:the parameters of C18O clumps}
\end{deluxetable*}
\end{longrotatetable}
